UDO: Universal Database Optimization using Reinforcement Learning

UDO is a versatile tool for offline tuning of database systems for specific workloads. UDO can consider a variety of tuning choices, reaching from picking transaction code variants over index selections up to database system parameter tuning. UDO uses reinforcement learning to converge to near-optimal configurations, creating and evaluating different configurations via actual query executions (instead of relying on simplifying cost models). To cater to different parameter types, UDO distinguishes heavy parameters (which are expensive to change, e.g. physical design parameters) from light parameters. Specifically for optimizing heavy parameters, UDO uses reinforcement learning algorithms that allow delaying the point at which the reward feedback becomes available. This gives us the freedom to optimize the point in time and the order in which different configurations are created and evaluated (by benchmarking a workload sample). UDO uses a cost-based planner to minimize reconfiguration overheads. For instance, it aims to amortize the creation of expensive data structures by consecutively evaluating configurations using them. We evaluate UDO on Postgres as well as MySQL and on TPC-H as well as TPC-C, optimizing a variety of light and heavy parameters concurrently.

==> deprecated/analysis.tex <==
\section{Theoretical Analysis}
\label{sec:analysis}

In this section, we prove convergence of Dealyed-UCT, and UDO framework using it for solving both heavy and light parameter UDO MDPs. We use regret~\citep{ucbv} as the performance metric for convergence. Given a time horizon $T$, regret $\reg_T$ is the sum of differences between the performance of the optimal configuration and the configuration achieved by the algorithm at any time step $t \leq T$. If the expected regret of an algorithm grows sublinearly with horizon $T$, it means the algorithm asymptotically converges to optimal configuration as $T \rightarrow \infty$.
% We discuss several reinforcement leaning algorithm here and provide the regret bound for the aforementioned two level reinforcement learning algorithm. We utilize the delay UCT and delay EXP3 tree search as the underlying delay reinforcement learning model. 

\subsection{Delayed-UCT}
% It is well-known that the UCT algorithm balances between exploration and exploitation in a principled manner that results in probabilistic guarantees. However, the traditional UCT algorithm has to update the reward of the selected actions at each round. \cite{} proposes a UCB manner selection strategy for online algorithm under the delayed feedback. We applied this selection strategy in the Monte Carlo Search Tree, and proposed the delay UCT algorithm. In the delay UCT tree, the reward of each tree node is not updated immediately. Instead, the reward information of each tree node can be updated after $d$ episodes from its selection, where $d$ is the maximal delay time as the input parameter.
\begin{lemma}[Regret of delayed-UCB-V]\label{thm:delayed-ucbv}
For any $T \geq 1$, the expected regret of delayed-UCB-V with delay $\tau$ is bounded by
\begin{align*}
    \mathbb{E}[\reg_T] \leq 10 \sum_{i: \Delta_i > 0} \left[ \left( \frac{\sigma_i^2}{\Delta_i} + 2b \right) \log T + \tau \Delta_i. \right]  
\end{align*}
Here, $\sigma_i^2$ is the variance of rewards for action $i$, $\Delta_i$ is the difference in expected rewards of the optimal action and action $i$, and $b>0$.
\end{lemma}
\textit{Proof sketch:} Following the proof of Theorem 7~\citep{Joulani2013a}, we decompose the expected regret of delayed-UCB-V in two terms. First term is the regret term appearing due to use of UCB-V itself. The second term is due to the error in computed statistics due to the delayed feedbacks. We can bound them individually using the UCB-V regret bound~\citep{ucbv} and delay times the suboptimality of rewards of all the actions, i.e. $\tau \sum_{i} \Delta_i$. By combining these, we obtain that the expected regret of delayed-UCB-V is $O(\log T + \tau)$.


\deba{For the next proof, we have to change a few stuffs in delayed-UCT. First is making the B value infinity for unvisited states. Second is modifying the selection process to $b_{p}(t) = \min\{\text{UCB-V equation for conf at }(p) + \rho^{depth(p)}, \max_{c \in C(p)} b_p(t)\}$. This framework of MCTS is called Hierarchical Optimistic Optimization (HOO)~\citep{bubeck2011a}.}

\begin{theorem}[Estimation Bias of Delayed-UCT]\label{thm:delayed-uct}
For a performance metric smooth around the optimal configuration, the error in the expected value of any state $s$ as estimated by delayed-UCT is bounded by $O\left(\left[\frac{\tau + \log T}{T}\right]^{1/(d+2)}\right)$ for a delay $\tau > 0$, horizon $T$, and $1/3$-near-optimality dimension $d$ of $f$. Typically, $d$ is upper bounded by the number of parameters.
\end{theorem}
\textit{Proof sketch:} The error in estimated expected reward of a given configuration at time $T$ is $r_T(c) = \frac{1}{T}\mathbb{E}[R_T(c)]$. By generalising Theorem 6 in~\citep{bubeck2011a}, we obtain that if an optimistic bandit algorithm with expected regret bound $O(g(T))$ is used in HOO framework, $\mathbb{E}[R_T(c)] \leq O(T^{\frac{d+1}{d+2}}(g(T))^{1/(d+2)})$. Now substituting $g(T)$ with Lemma~\ref{thm:delayed-ucbv} and using relation between error and regret, we obtain that $r_T(c) = O\left(\left[\frac{\tau + \log T}{T}\right]^{1/(d+2)}\right)$ for delayed-UCT.

This shows that the error in estimating the expected performance (or reward) of a configuration using delayed-UCT converges at the rate $O\left(\left[\frac{\tau + \log T}{T}\right]^{1/(d+2)}\right)$, where $T$ is the number of times the configuration is evaluated.
% \subsection{Delay EXP3}
% Delay EXP3 selection strategy is proposed in \cite{} for the delay multi-arm bandit problem. Compared with UCB, it adopts the probabilistic policies instead of deterministic policies, 
% % The advantage of EXP3 compared with UCB selection strategy is that 

% \begin{theorem}
% For the delay EXP3 algorithm, the expected regret is bounded by $O()$
% \end{theorem}

\subsection{UDO}
As we have obtained the estimation bias of the delayed-UCT algorithm, now we can derive bound on UDO algorithm that applies delayed-UCT at two levels with two different delays.

\begin{theorem}
Regret bound: If we plugin the delay UCT as the delay reinforcement learning model, and UCT as the non-delay reinforcement learning model, the expected regret of the UDO is bounded by $O\left(T_h^{(d+1)/(d+2)} (\log T_h + \tau + \epsilon(T_l))^{1/(d+12)}\right)$. Here, $\epsilon(T_l) = \left(\frac{T_l}{\log T_l}\right)^{-1/(d+12)}$.
% $O(\log(N_1) + \log(N_2))$.
\end{theorem}
\textit{Proof sketch:} The proof for UDO is similar to bounding regret for delayed-UCT on the heavy parameters' configuration space, where the rewards are observed with some estimation error. 
We prove the regret bound in three steps:\\
a. Like delayed-UCT proof, we reduce UDO regret to that of the delayed-UCB-V regret but with estimation error.\\
b. We decompose the regret of delayed-UCB-V in three error terms due to UCB-V, delay, and estimation error for light parameters.\\
c. We plug-in regret bound of UCB-V, delay times suboptimality of expected reward of actions, and biased induced by delayed-UCT with $\tau=0$ as obtained for light parameter MDPs.

% We prove the convergence rate of our algorithm
% \begin{theorem}
% Convergence speed: If we plugin the delay UCT as the delay reinforcement learning model, and UCT as the non-delay reinforcement learning model, the algorithm coverage to the best configuration after episode.
% \end{theorem}
Thus, deviation in the expected performance of the configuration returned by UDO from optimal configuration is $O\left(\left[\frac{T_h}{\log T_h + \tau + \epsilon(T_l) }\right]^{-1/(d+2)}\right)$. Here, $T_h$ and $T_l$ are the number of steps allotted for the heavy and light parameters respectively. 







==> deprecated/demo_setup.tex <==
\section{Demonstration Setup}
\label{sec:demonstration}

Our demonstration consists of two parts. First, we give participants the opportunity to compare alternative configurations against the ones found by UDO. Second, we give participants a chance to visualize convergence of UDO for different parameters, based on pre-recorded traces. 

\textbf{Competition.} We will provide participants with access to an EC2 machine on which the TPC-H benchmark is installed. We will point audience members to a public document in which they can register for access during 30 minutes time slots. We will provide registered participants with the login details, a list of parameters considered by UDO, and the final performance numbers achieved. Visitors are free to try out different configurations, also installing tuning tools of their choice. In case of significant changes, we will be able to restore the defaults quickly via a stored EC2 AMI. Participants may send us their best performing configuration. We will benchmark the configuration ourselves and maintain a public ``high-score list'' with achieved performance results.

\textbf{Visualization.} Audience members may gain insights into how UDO works internally, using a visualization tool. To save time, we will provide pre-recorded optimization traces for TPC-C on MySQL and Postgres for download, together with the visualization tool. The visualization tool allows users to select subsets of parameters to visualize, and shows a video illustrating UDO's convergence over time (in addition to statistics such as reward values, visit frequencies, and UCT search tree growth). Figure~\ref{fig:screenshot} shows a screenshot.

\begin{comment}
In our demonstration, we will show: a) UDO selects better configurations compared to baselines; b) UDO selects better configurations than human experts. We will provide some Amazon EC2 machines on which UDO and baselines are installed. Users can try different baselines on those EC2 machines or they can try to find better configurations by themselves.

% We also provide videos which demonstrate how UDO converges to optimal configuration gradually.

% Visitors can access laptops on which all the baselines and UDO are installed. Visitors can choose the whole configuration space or select configuration sub-spaces. Visitors have access to Amazon EC2 machines on which UDO and baselines are installed.

% \textbf{Visualization} Our visualization tool allows users to choose log files generated by UDO, and parameters to visualize.
% % select their interested configurations and show how does the tree grows. 

\textbf{Comparison with human experts.} Visitors can tune the TPC-C/TPC-H benchmarks by themselves to achieve the best performance. For the transaction template optimization, we provide the GUI interface which decomposes code units and identifies the constraints between those units. They can reorder those code units without violating the semantics. For database indexes, the interface lists all the potentially useful indexes after analyzing transaction queries. Users can select indexes to create. For the system tuning parameters, the GUI interface lists all parameters and valid values, users can try to figure out what is the optimal setting.

\textbf{Comparison with baselines.} Visitors can run the aforementioned baselines on the same machines. Convergence times can be elevated, depending on the settings. Hence, we offer visitors the opportunity to leave their mail address. After running experiments in the Cloud, visitors will be notified via email after their results are ready. We also prepare some videos which show how UDO performances compared with those baselines.

\textbf{Visualization} Our visualization tool allows users to choose log files generated by UDO, and parameters to visualize. Figure \ref{fig:index} shows the tuning parameters that can be visualized for the TPC-H benchmark. Tuning parameters can be visualized for the ~\ref{fig:idxtree}. Figure ~\ref{fig:ordertree} shows the expansion of the light search tree for the payment transaction after 10 micro-episodes. The size of the tree node varies based on its number of visits. The accumulated average reward of each path is marked near the leaf nodes. 
\end{comment}

% We visualize search trees which allows visitors to gain insights on how heavy and light search trees grow and expand. Our system keep records of the growth of the tree and 

% For the learning procedure, we visualize the approximation mistake and the expansion of different search trees. Figure ~\ref{fig:decompose} shows the evolution of the simulation gap (i.e., the distance between our enabled heavy configurations and the sampled configuration in the next macro-episode). Figure ~\ref{fig:index} shows the expansion of the search tree for the payment transaction after sampling 10 times. Figure ~\ref{fig:index} shows the expansion of one index tree after sampling 10 times. The legend shows the details of the corresponding tree node, e.g., the code unit number or the detailed index information. The size of the tree node varies based on its number of visits. The accumulated average reward of each path is marked near the leaf nodes. 

%Visitors run UDO for two minutes on the TPC-C benchmark atop of MySQL (v5.7.29) and compete against other results on 10 Amazon EC2 instances.


% \textbf{Comparison with human experts.} Visitors can tune the TPC-C benchmark by themselves to achieve the best performance. For the transaction template optimization, we provide the GUI interface which decomposes code units and identifies the constraints between those units. They can reorder those code units without violating the semantics. For database indexes, the interface lists all the potentially useful indexes after analyzing transaction queries. Users can select indexes to create. For the system tuning parameters, users can choose among all valid values.

% \textbf{Comparison with baselines.} Visitors can run the aforementioned baselines on the same machines. Convergence times can be elevated, depending on the settings. Hence, we offer visitors the opportunity to leave their mail address. After running experiments in the Cloud, visitors will be notified via email after their results are ready. We also prepare some videos which show how UDO works compared with those baselines.

\begin{figure}
    \centering
       \includegraphics[width=0.375\paperwidth]{fig/idx tree.png}
    \caption{Screenshot of UDO visualization tool.}
    \label{fig:screenshot}
\end{figure}

\begin{comment}
\begin{figure}
    \centering
    % \subfigure[Overview of indexes]{
    %     \includegraphics[width=0.35\paperwidth]{fig/system.png}
    %     \label{fig:index}
    % }
    % \hfill
    \begin{subfigure}[Expansion of search tree for selected indexes] {
        \centering
        \includegraphics[width=0.375\paperwidth]{fig/idx tree.png}
        \label{fig:idxtree}
    } \end{subfigure}
    ~
    \centering
    \vspace{-1em}
    \begin{subfigure}[Expansion of the payment reorder search tree] {
        \centering
        \includegraphics[width=0.15\paperwidth]{fig/parameter tree.png}
        \label{fig:ordertree}
        % \caption{Expansion of the payment code reorder search tree}
    } \end{subfigure}%
    \caption{Expansion of different search trees}
    \vspace{-1.5em}
\end{figure}
\end{comment}



==> deprecated/evaluator.tex <==
% \section{Algorithm}
% \label{sec:algorithm}
% To decrease the index creation overhead, we propose a two approach search tree approach, shown in ~ Alg \ref{alg:two_level}.


% \begin{algorithm}[t!]
% \caption{Delay EXP3 MCTS}
% \renewcommand{\algorithmiccomment}[1]{// #1}
% \begin{small}
% \begin{algorithmic}[1]
% \State \Comment{Sample configurations from tree node $T$ at timestamp $i$}
% \Function{SAMPLE}{$T, i$}
%     \State \Comment{$T$ does not have any children}
%     \If{$T.children = \emptyset$}
%         \State c = \Call{ROLL\_OUT}{$T$}
%         \State Return c
%     \Else
%         \State \Comment{Select an action from the current node}
%         \State $a$ = \Call{SELECTION}{$T$}
%         \State \Comment{Recursive sample from children}
%         \State Return $c \circ$ \Call{SAMPLE}{$T_r$}
%     \EndIf
% \EndFunction
% \Function{SELECTION}{$T_r$}
%     \State Select a child node $a$ according to distribution $\vec{p}_i$
% \EndFunction
% \State \Comment{Update the search tree from root to leaves}
% \Function{UPDATE}{$T_l, r_l$}
%     \State 
% \EndFunction
% %  m, s_m, i, 
% \State \Comment{$m$ is the selected action of the node $T$, $l$ is the current loss}
% \Function{UPDATE\_NODE}{$T, l, m$}
%     % \State $\hat{l}_{s_m|i} = l_{s_m|i} / \vec{p}_t(m)$
%     \State $\hat{l}= l / \vec{p}_t(m)$
%     \State $\widetilde{w}_i^n (m) = \vec{p}_i^{n-1}(m) \exp(-\eta \min\{\delta_1, \hat{l}\})$
%     % \exp(-\eta \min\{\delta_1, \hat{l}_{s_m|i}\})$
%     \State $w_i^n (m) = \max \{\widetilde{w}_i^n (m)/ \sum_{j=1}^{|A|} \widetilde{w}_i^n (j), \frac{\delta_2}{|A|} \}$
%     \State $\vec{p}_i^{n}(m) = w_i^n (m) / \sum_{j=1}^{|A|} w_i^n (j)$
%     \If{$T_n = \emptyset$}
%         \State \Call{UPDATE\_NODE}{$T_m, l, m.next$}
%     \EndIf
% \EndFunction
% \end{algorithmic}
% \end{small}
% \end{algorithm}


% \section{REORDER CONFIGURATIONS}

% \section{PLANING}

\section{Evaluator}
The main procedure for the evaluator is to determine which configurations to evaluate and the evaluation order of the selected configurations.


\begin{algorithm}[t!]
\caption{Evaluator}
\label{alg:evaluator}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} A configuration pool $P_h$
\State \textbf{Output:} the evaluation plan
\Function{Evaluation}{$P_h$}
    \State $P_h^s \gets $ \Call{EvaluatorManager.DecideConfigurations}{$P_h$}
    \State $P_h^o \gets$ \Call{EvaluatorPlan.DecideEvaluateOrder}{$P_h^s$}
    \State \Return $P^o_h$
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

\subsection{Evaluation Manager}

In this section, we introduce how does the evaluation manager select the configurations to evaluate from the configuration pool $P_h$ at each timestamp.

\subsubsection{Offline Selection}

Given the maximal delay tolerance $d$ of the reinforcement learning algorithm, the offline selection strategy for the evaluation manger is to not evaluate configurations in $P_h$ when the size of the configuration pool $P_h$ is less then $d$ and evaluate all configurations in that pool $P_h$ when the size of the configuration pool $P_h$ exceeds $d$. To be more specific, give the maximal delay tolerance $d$ of reinforcement learning algorithm, with the offline selection strategy, we pass this configuration to evaluation planner until the size of configuration pool $P_h$ reaches to $d$. Then we clear the configuration pool $P_h$. 

% a simple strategy is that we can collect the sampled configurations into the configuration pool $P_h$ until the size of configuration pool $P_h$ reaches to $d$. Then we feed this configuration list into the evaluation planner and clear the configuration pool $P_h$. 

% selection configurations batch by batch.

\subsubsection{Online Selection}

The online selection strategy is shown in Algorithm \ref{alg:evaluator_manager}. Suppose the delay tolerance given by the reinforcement leaning algorithm is denoted as $d$, for a specific configuration $c$ generated at timestamp $t$, UDO does not consider to evaluate this configuration until the timestamp $t + \frac{d}{e}$. Instead it calculates the minimal evaluation cost $c_{\min}$ of that configuration $c$ during time interval $[t, t + \frac{d}{e}]$. After the timestamp $t + \frac{d}{e}$, UDO calculates the evaluation cost of $c$ at each timestamp and if there exists a timestamp producing the smaller cost than the minimal cost $c_{\min}$, UDO adds the configuration $c$ into the evaluation configuration list. Otherwise, the configuration $c$ will be evaluated at the timestamp $t+d$. UDO employs this selection strategy for all configurations in the configuration pool $P_h$.

% The online procedure is formalized as, at each time $t$, the algorithm has to evaluate the configuration generated at time $t - \Delta t$ and decides whether to evaluate the pending configurations generated after time $t - \Delta t$. Thus it is crucial to estimate the benefit of 

\begin{algorithm}[t!]
\caption{Evaluator manager with a non-fixed delay}
\label{alg:evaluator_manager}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
% \Function{DecideConfigurations}{$P_h$}
%     \If{$P_h.size = d$}
%         \State \Return $P_h$
%     \Else
%         \State \Return $\emptyset$
%     \EndIf
% \EndFunction
\State \textbf{Input:} A configuration pool $P_h$, the current timestamp $t$, the maximal delay tolerance $d$ and the fraction of training time $r$
\State \textbf{Output:} the evaluation plan
\Procedure{DecideConfigurations}{$P_h, t, d, r$}
    \State \Comment{Calculate the saving cost of each configuration}
    \State $P_h^s \gets []$
    \For{$\langle c_h, t_h \rangle \in P_h$}
        \State \Comment{Check the sampled time $t_h$ of the configuration $c_h$}
        \If{$t = t_h + d$}
            \State \Comment{Current configuration $c_h$ has to be evaluated}
            \State $P_h^s \gets P_h^s \circ c_h$
        \Else
            \State \Comment{Cost of evaluating configuration $c_h$ at current timestamp}
            \State $c \gets$ \Call{CostSavings}{$P_h^s, c_h$}
            \If{$t \leq c_h + d r$}
                \State \Comment{Collect the min saving cost during the $d r$ slot}
                \State $c_{\min}(c_h) \gets \min(c, c_{\min}(c_h))$
            \ElsIf{$c \leq c_{\min}(c_h)$}
                \State \Comment{Decide to evaluate $c_h$ at that timestamp}
                \State $P_h^s \gets P_h^s \circ c_h$
            \EndIf
        \EndIf 
    \EndFor
\EndProcedure
\end{algorithmic}
\end{small}
\end{algorithm}

\subsection{Evaluation Planner}

Now, we introduce the main task of the evaluation planner, given a list of heavy configuration $C_h$, it decides the min cost order to build those heavy
configurations minimizing the switching overhead.

% To increase the sample efficiency, the key is to decrease the switching overhead of heavy parameters. 

% We propose several algorithms to incrementally construct the heavy parameters aiming to decrease the switching overhead. 

% We formalize our reorder problem as follows, given the maximal delay tolerance time $\Delta t$, at each timestamp $t$, we receive a configuration $c_t$ generated by the delay reinforcement learning model and decide which configurations are evaluated at the current stage (notice that the configurations generated at timestamp $t - \Delta t$ must be evaluated. We consider both online algorithm and offline algorithm to solve this problem. 

% \subsubsection{Offline algorithm}

We formalize this procedure as follows, given a configuration list $C_h = \{ c_1, c_2, \cdots, c_l \}$ with length $l$ and a $\text{cost}$ function mapping from a specific configuration to its build/drop cost, our goal is to find a permutation of configuration set $C$, denoted as $\bar{C} = \{ \bar{c}_1, \bar{c}_2, \cdots, \bar{c}_l \}$, such that the total cost of $\bar{C}$, $\sum_{t=1}^{l} \bar{c}_t - \sum_{t=1}^{l-1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$ is minimized. This problem is same as maximizing the overlapping cost, $\sum_{t=1}^{l - 1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$. 

% from timestamp $t = 0, 1, \cdots, \Delta t$ and $\text{cost}$ is a function mapping from specific configurations to their build/drop costs.. Our goal is to 

% We simplify the previous procedure to the following offline procedure, instead deciding which configurations to evaluate, we gather continuous configurations for the time interval $\Delta t$, and find the min cost order for all those heavy configurations. For example, the reinforcement learning algorithm generates configurations $C = \{ c_0, c_1, \cdots, c_{\Delta t} \}$ from timestamp $t = 0, 1, \cdots, \Delta t$ and $\text{cost}$ is a function mapping from specific configurations to their build/drop costs.. Our goal is to find a permutation of configuration set $C$, denoted as $\bar{C} = \{ \bar{c}_0, \bar{c}_1, \cdots, \bar{c}_{\Delta t} \}$, such that the total cost of $\bar{C}$, $\sum_{t=0}^{\Delta t} \bar{c}_t - \sum_{t=0}^{\Delta t - 1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$ is minimized. This problem is same as maximizing $\sum_{t=0}^{\Delta t - 1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$.

% \subsubsection{NP-complete proof}

% We reduce this problem to the shortest common superstring problem to prove its NP-completeness. The shortest common superstring problem is defined as, given a alphabet $\Sigma$ and a set of $n$ strings $S =\{s_1, s_2, \cdots, c_n\} \subset \Sigma$, we want to find the
% shortest string $s$ that contains $s_i, \forall i = \{1, 2, \cdots, n\}$ as a substring. Suppose we are given a min cost configuration solver and a set of $n$ strings $S$, we initialize the cost of all letters in the alphabet as 1.  

\begin{theorem}
The aforementioned min cost problem is a NP-complete problem.
\end{theorem}

\begin{proof}
We reduce this problem to Hamiltonian path problem. Given a graph $G$ of $n$ vertices and a min cost order solver, we represent each vertex $i$ of the graph $G$ to one configuration set $c_i$. And if there exist one edge between vertex $i$ and $j$, we construct the set $c_i$ and $c_j$ which have one overlap configuration. And if there does not exist one edge between vertex $i$ and $j$, the constructed set $c_i$ and $c_j$ does not have any overlap configurations. Then we generate a list of configurations $\{c_0, c_1, \cdots, c_n\}$ using the given graph. Then we feed this configuration list into our min cost order solver with the cost function mapping each configuration to one. Then we obtain a permutation order of the configuration list $C$. We traverse the graph using this obtained order, if we generate a path finally, the generated path is a valid Hamiltonian path, otherwise the graph does not exist any Hamiltonian path. 
% Now, we are ready to prove the completeness and soundness of this reduction.
% Completeness: we argue that a "yes" instance of Hamiltonian path is transformed into  a "yes" instance of the min cost order problem via the previous reduction.  
% Soundness: we argue that a "yes" instance of the min cost order problem must correspond to a "yes" instance of Hamiltonian path problem.
\end{proof}

\subsubsection{Greedy approach}
We introduce a greedy approach to approximately solve the min cost order problem shown in Algorithm ~\ref{alg:greedy_approach}. This approach initializes the order $o$ for the first two configuration as $[0, 1]$. Then the greedy approach iterates from the third configuration to last configuration, and at each step, it find the insert position which leads to the maximal overlapping cost for the current order $o$. After processing all configurations, it return the final order $o$.

\begin{algorithm}[t!]
\caption{The greedy approach for min cost order problem}
\label{alg:greedy_approach}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} A configuration list $P_h^s$ with length $l$
\State \textbf{Output:} Min cost order
\Function{GreedyMinCostOrder}{$P_h^s$}
\State $o \gets [0, 1]$
% \State $c =$ \Call{cost}{$L[0]$} +  \Call{cost}{$L[1]$} - \Call{cost}{$L[0] \cap L[1]$}
% \State \Comment{Initialize the cost}
% \State $c \gets cost(C_h[0]) + cost(C_h[1]) - cost(C_h[0] \cap C_h[1])$
% \State $c \gets cost(P_h^s[0] \circ P_h^s[1])$
\State \Comment{Consider configurations from $2$ to $l$}
\For{$i \gets 2$ to $l$} 
    \State \Comment{Pick up the position $p$ which has the maximal overlap cost}
    % \State $p \gets \arg \min_{0 \leq j \leq i} \{ c - cost(C_h[j-1] \cap C_h[j]) + cost(C_h[j - 1] \cap C_h[i]) + cost(C_h[j] \cap C_h[i]) \}$ 
    \State $sc \gets $ \Call{cost}{$P_h^s[o[j - 1]] \cap P_h^s[o[i]]$} + \Call{cost}{$P_h^s[o[j]] \cap P_h^s[o[i]]$}
    \State $p \gets \arg \max_{0 \leq j \leq i} sc -$ \Call{Cost}{$P_h^s[o[j - 1]] \cap P_h^s[o[j]]$}
    % \{ c - cost(C_h[j-1] \cap C_h[j]) + cost(C_h[j - 1] \cap C_h[i]) + cost(C_h[j] \cap C_h[i]) \}$ 
    % \State $c_{\min} = 0$
    % \State $p = 0$
    % \For{$j \gets 0$ to $i$} 
    %     \State $c_j = c$ - \Call{cost}{$L[j-1] \cap L[j]$} + \Call{cost}{$L[i]$} - \Call{cost}{$L[j - 1] \cap L[i]$} - \Call{cost}{$L[j] \cap L[i]$} 
    %     \If{$c_{\min} < c_j$}
    %         \State $c_{\min} = c_j$
    %         \State $p = j$
    %     \EndIf
    % \EndFor
    % \State $c \gets c - cost(C_h[p-1] \cap C_h[p]) + cost(C_h[p - 1] \cap L[i]) + cost(C_h[p] \cap C_h[i])$
    \State \Comment{insert into $i$-th unit into the position $p$}
    \State $o.insert(i, p)$
\EndFor
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

\junxiong{Notation consistency of $C$ and $P$}

\subsubsection{Dynamic programming approach}
We propose a dynamic programming algorithm to solve the min cost order problem, shown in ~\ref{alg:dp_approach}.
% We generate the powerset of the permutation unit, for example if the delay time $\Delta t = 5$, the generated set is the powerser of $\{1, 2, 3, 4, 5\}$. We iterate the generated powerset by increasing the cardinality and calculate the min cost 
For a given configuration $P_h^s$ with length $l$, we construct the cost array for orders with length $2^h$ where $h \leq l$ and $h \in \mathbb{N}$ from bottom to up. At $i$-iteration, the algorithm calculates the cost of orders with length $2^i$ using the cost information from the bottom level $2^{i-1}$. For a order $o$, the algorithm splits it into a list of orders where each order has a length with power of two. For example, an order $[1, 2, 3, 4, 0, 6, 7, 5]$ is split into $[1, 2, 3, 4]$ and $[0, 6, 7, 5]$ to calculate the cost information and it is obvious that the cost of $[1, 2, 3, 4]$ and $[0, 6, 7, 5]$ is calculated in the previous iterations. Finally, the algorithm enumerate of possible order for this configuration list $P_h^s$ and use the previous cost information to find the min cost order.

% subsets with length $2^h$ where $h \leq l$ and $h \in \mathbb{N}$ from bottom to up.

% $O(2^n)$

% $O(2^n)$

% We formalize it as a dynamic programming  

\begin{algorithm}[t!]
\caption{The dynamic programming approach for min cost order problem}
\label{alg:dp_approach}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} A configuration list $P_h^s$ with length $l$
\State \textbf{Output:} Min cost order
\Function{DPMinCostOrder}{$P_h^s$}
% \State \Comment{Generate all permutations of subsets of the sequence from $1$ to $l$}
% \State $L \gets \mathcal{P} (\{1, 2, \cdots, l\})$
% \State $L_p \gets $ \Call{Prune}{$L$}
% \State \Comment{Sort the list $L$ by their cardinality in a ascending order}
% \State $L_o \gets$ \Call{Sort}{L_p}
% \For{$s \in S_o$}
%     \State 
%     % \State \Comment{Calculate the cost of an order $s$ by considering all position insert point}
%     % \For{$s \in S_o$}
%     % \EndFor
% \EndFor
\State $O \gets \{0, 1, \cdots, l\}$
\State $C([i]) \gets $ \Call{Cost}{$P_h^s[i]$}
\State $k \gets \arg \max_k \{2^k \leq l, k \in \mathbb{N}\}$
\For{$i \gets 1$ to $k$}
\State \Comment{Generate all permutations for subsets of $O$ with length $2^k$}
\State $O_i \gets$ \Call{GeneratePermutation}{$O, 2^k$}
\For{$o \in O_i$}
    % \State \Comment{Calculate the cost of an order $o$}
    \State  $C(o) \gets$ \Call{CaculateCost}{$P_h^s, o, C$}
    % \State \Comment{Each list in $S$ has a length power of 2}
    % \State $S \gets$ \Call{GeometrySplit}{$o$}
    % \State $C(o) \gets \sum_{s \in S} C(s) - \sum_{j=1}^{k} $ \Call{Cost}{$P_h^s[S[j].{last}] \cap P_h^s[S[j+1].{first}] $}
\EndFor
\EndFor
\State \Comment{Generate all permutations of the sequence from $1$ to $l$}
\State $P \gets$ \Call{GeneratePermutation}{$O, l$}
\State \Return $\arg \max_{p \in P} $ \Call{CaculateCost}{$P_h^s, p, C$}
\EndFunction
\State \textbf{Input:} A configuration list $P_h^s$, a order $o$ and the previous cost $C$
\State \textbf{Output:} Cost of order
\Function{CaculateCost}{$P_h^s, o, C$}
    \State \Comment{Calculate the cost of each permutation}
    \State $S \gets$ \Call{GeometrySplit}{$o$}
    \State \Comment{Calculate the saving cost}
    \State $sc \gets \sum_{j=1}^{k} $ \Call{Cost}{$P_h^s[S[j].{last}] \cap P_h^s[S[j+1].{first}]$}
    \State \Return $\sum_{s \in S} C(s) - sc$
    % \State $C(o) \gets \sum_{s \in S} C(s) - sc$
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

\subsubsection{Integer programming approach}

We formalize it as an integer programming problem as follows, we use $x_{ij}$ to denote the $i$-th unit is reordered to the $j$-th place. If $x_{ij} = 1$, the $i$-th unit is recorded to the $j$-th place, otherwise it is not reordered to $j$-th place. Then the min cost problem can be represented as, 
% And we formalize it as a linear programming problem.

% \begin{equation}
% \begin{split}
%     \sum_{i=1}^{d} x_{ij} & = 1 \\
%     \sum_{j=1}^{d} x_{ij} & = 1 \\
% \end{split}
% \end{equation}

\begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum_{i=1}^{\Delta t} \sum_{j=1}^{\Delta t - 1}\sum_{k=1}^{\Delta t} x_{ij} x_{k (j+1)} \text{cost}(c_{i} \cap c_{k}) &\\
\text{subject to}& \displaystyle\sum_{i=1}^{\Delta t} x_{ij}  = 1,  &j=1 ,..., \Delta t\\
& \displaystyle\sum_{j=1}^{\Delta t} x_{ij} = 1,  &i=1 ,..., \Delta t\\
\end{array}
\end{equation*}

Since $x_{ij}$ is a binary variable, after applying the linearity, the previous min cost problem can be rewritten,

\begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle
\sum_{i=1}^{\Delta t} 
\sum_{j=1}^{\Delta t - 1}
\sum_{k=1}^{\Delta t} z_{ijk}
\text{cost}(c_{i} \cap c_{k}) 
&\\
\text{subject to}& 
\displaystyle z_{ijk} \leq \frac{1}{2} (x_{ij} + x_{k (j+1)}) \\
& \displaystyle\sum_{i=1}^{\Delta t} x_{ij}  = 1,  &j=1 ,..., \Delta t\\
& \displaystyle\sum_{j=1}^{\Delta t} x_{ij} = 1,  &i=1 ,..., \Delta t\\
\end{array}
\end{equation*}


% \subsection{Online algorithm}
% The online procedure is formalized as, at each time $t$, the algorithm has to evaluate the configuration generated at time $t - \Delta t$ and decides whether to evaluate the pending configurations generated after time $t - \Delta t$. Thus it is crucial to estimate the benefit of 

% \begin{algorithm}[t!]
% \caption{The online approach for min cost order problem}
% \label{alg:online_approach}
% \renewcommand{\algorithmiccomment}[1]{// #1}
% \begin{small}
% \begin{algorithmic}[1]
% \State \textbf{Input:} A configuration list $L$, 
% \State \textbf{Output:} Min cost evaluating order
% \end{algorithmic}
% \end{small}
% \end{algorithm}


% We can plugin in any delay reinforcement learning model for heavy parameters. The delay reinforcement learning model should provide three functions, \textbf{SAMPLE} to generate samples, \textbf{UPDATE} to update the statistics information of actions, \textbf{OPT} to retrieve a best policy.

% After the delay reinforcement learning model picks up $d$ samples. UDO decides the evaluating order via \textbf{MINCOSTORDER} function discussed in the next section. During each episode, we construct the non-delay reinforcement learning model for light parameters. The reinforcement learning model of light parameters generates one trajectory using the current policy until reaching to a terminate state. After that, UDO switches to the selected configurations and evaluates the performance of the selected configurations. The light parameter reinforcement learning model updates its policy information using simulation results. After $N_2$ episode for the bottom level, we retrieve the best configuration and its performance. Then we update the delay reinforcement learning model using the best performance found at the bottom level.




% With the episodic MDP for the naive UDO, it is straightforward to propose the following algorithms. 

% \junxiong{question about the reward scaling $[0, 1]$}



% \paragraph{MCTS for the naive UDO} We tackle this problem using Monte Carlo Tree search under the naive UDO MDP, in which each tree node represents a state indicating the current configuration and each edge represents an action showing selected change of the current configuration. At each episode, we traverse the search tree from root and pick up one action at each step until reaching to a leaf. Then we switch to selected actions, which may include heavy configurations and light configurations. Then our system UDO runs the given workload and calculate the reward based on the obtained performance. UDO uses UCB-V as the selection policy to balance the exploration and exploitation, which selects the child node $c$ maximizing the formula $r_c+\sqrt{2.4 \sigma_c^2 \frac{\log(v_p)}{v_c}} + \frac{3 b \log(v_p)}{v_c}$ where $r_c$ is the average reward and $\sigma_c^2$ is the variance of reward, $v_p$ and $v_c$ are the number of visits for child and parent node, proposed in \cite{}.

% % \paragraph{Limitation of the naive UDO}
% However, frequently switching of heavy configurations (e.g., creating or dropping indices) decreases exploration frequency, thereby leading to slow convergence. In fact, reinforcement learning is considered most effective in scenarios where a high frequency of trials (i.e., action invocations) can be achieved. However, with this simple idea, we face the problem that changing heavy parameters prevents us from achieving high frequencies.

% To improve the sample efficiency, we separate the parameters into heavy and light parameters and propose a two level episode procedure presented in Algorithm ~\ref{alg:two_level}.



% Finally, the reinforcement learning model updates its reward using its obtained performance. 

% determines actions until reaching to the terminate state, generates one trajectory using the current policy 

% generates $d$ samples. 

% UDO decomposes a search tree into a light parameter search tree and a heavy parameter search tree.

% \junxiong{highly level approach}

% \junxiong{evaluator, and evaluation policy}

% \junxiong{evaluator, heavy coniguration, argmax}


% \begin{algorithm}[t!]
% \caption{Two level approach of UDO using the delay reinforcement learning model}
% \renewcommand{\algorithmiccomment}[1]{// #1}
% \begin{small}
% \begin{algorithmic}[1]
% % \State \Comment{Optimize transactions in the given configuration space}
% % \State \Comment{$C$ is the given configuration spaces, $L_t$ is the macro episode}
% % \State \Comment{$M_t$ is the micro episode}
% % \Procedure{UniversialOptimization}{$C, L_t, M_t$}
% \State \textbf{Input:} Configuration spaces $C$, number of episode $N_1$ for heavy parameters, number of episode $N_2$ for light parameters, the maximal delay tolerance $d$
% \State \textbf{Output:} the best obtained configuration
% \State \Comment{Divide the configuration space $C$ into heavy configurations $C_H$ and light configurations $C_L$}
% \State $C_H, C_L \gets$ \Call{SplitParameter}{$C$}
% \State $M_H$ = \Call{ConstructDelayRLModel}{$C_H$}
% \While{$t_1 \leq N_1$}
%     % \State $d$ = \Call{DetermineDelaySample}{$t_1$}
%     \For{$i \gets 1$ \textbf{to} $d$}
%         \State $c_h^i$ = \Call{Sample}{$M_H$}
%     \EndFor
%     \State \Comment{Decide the order to evaluate $c_h^0, c_h^1, \cdots, c_h^d$}
%     \State $C_h^o =$ \Call{MinCostOrder}{$c_h^0, c_h^1, \cdots, c_h^d$}
%     \For{$i \gets 1$ \textbf{to} $d$}
%         \State $c_h^i = C_h^o[i]$
%         \State \Call{IncrementalBuildHeavyConfiguration}{$c_h^i$}
%         \State \Comment{Construct the tree of light configurations for current heavy configuration}
%         \State $M_L$ = \Call{ConstructRLModel}{$C_L$}
%         \While{$t_2 \leq N_2$}
%             \State \Comment{Sample from the RL model for light parameters}
%             \State $c_l$ = \Call{Sample}{$M_L$}
%             \State \Comment{Evaluate the performance of light parameters under the heavy parameters}
%             \State $r_l$ = \Call{Evaluate}{$c_l$}
%             \State \Comment{Update the RL model for light parameters}
%             \State \Call{Update}{$M_l, r_l$}
%         \EndWhile
%         \State \Comment{Obtain the best light parameter for current heavy parameter}
%         \State $c_l, r$ = \Call{Opt}{$M_L$}
%         \State \Call{Update}{$M_H, c_h^i, r$}
%     \EndFor
%     \State $t_1 \gets t_1 + d$
% \EndWhile
% \State \Comment{Return the best obtained configuration}
% \State $c_h, c_l, r$ = \Call{Opt}{$M_H$}
% % \EndProcedure
% \end{algorithmic}
% \end{small}
% \end{algorithm}

% Algorithm \ref{alg:two_level_online} shows a modification of two level reinforcement learning algorithm. Instead of evaluating the heavy configurations batch by batch, UDO initialize a configuration pool to collect the heavy configurations generated by the delay reinforcement learning model. At each episode, UDO adds the current sampled configuration to that configuration pool. UDO tests whether there exist a configuration which reaches to the maximal delay. If no configuration has to be evaluated, we continue this procedure, otherwise UDO decides heavy configurations to be created. Then, UDO applies the min cost algorithm to determine the evaluating order of those heavy configurations. Similarly, for each heavy parameter, UDO constructs the non-delay reinforcement learning model to learn the best light parameters under the given heavy parameters. The light parameter reinforcement learning model utilizes the stimulated trajectory and reward information to update its policy. After $N_2$ episode for the bottom level, we update the delay reinforcement learning model using the best performance found within the $N_2$ episode.

% % accumulates the heavy configurations until one configuration reaches to the maximal delay time. 

% \begin{algorithm}[t!]
% \caption{Two level approach of UDO using the delay reinforcement learning model and online order}
% \label{alg:two_level_online}
% \renewcommand{\algorithmiccomment}[1]{// #1}
% \begin{small}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Configuration spaces $C$, number of episode $N_1$ for heavy parameters, number of episode $N_2$ for light parameters, the maximal delay tolerance $d$
% \State \textbf{Output:} Best obtained configuration
% \State \Comment{Divide the configuration space $C$ into heavy configurations $C_H$ and light configurations $C_L$}
% \State $C_H, C_L \gets$ \Call{SplitParameter}{$C$}
% \State $P_H = \emptyset$
% \State $M_H$ = \Call{ConstructDelayRLModel}{$C_H$}
% \While{$t_1 \leq N_1$}
%     \State $c_h^{t_1}$ = \Call{Sample}{$M_H$}
%     \State $P_H = P_H \cup \{c_h^{t_1}\}$
%     \State \Comment{Check whether there exist a configuration satisfying delay deadline}
%     \If{$c_h^{t_1 - d} \in P_H$}
%         \State \Comment{Decide the configurations to evaluate}
%         \State $C_h =$ \Call{ConfigToEvaluate}{$P_H$}
%         \State \Comment{Decide the order to evaluate $c_h^0, c_h^1, \cdots, c_h^d$}
%         \State $C_h^o =$ \Call{MinCostOrder}{$C_h$}
%         \For{$i \gets 1$ \textbf{to} $d$}
%             \State $c_h^i = C_h^o[i]$
%             \State \Call{IncrementalBuildHeavyConfiguration}{$c_h^i$}
%             \State \Comment{Construct the tree of light configurations for   current heavy configuration}
%             \State $M_L$ = \Call{ConstructRLModel}{$C_L$}
%             \While{$t_2 \leq N_2$}
%                 \State \Comment{Sample from the RL model for light parameters}
%                 \State $c_l$ = \Call{Sample}{$M_L$}
%                 \State \Comment{Evaluate the performance of light parameters under the heavy parameters}
%                 \State $r_l$ = \Call{Evaluate}{$c_l$}
%                 \State \Comment{Update the RL model for light parameters}
%                 \State \Call{Update}{$M_l, r_l$}
%             \EndWhile
%         \State $c_l, r$ = \Call{Opt}{$M_L$}
%         \State \Call{Update}{$M_H, c_h^i, r$}
%     \EndFor
%     \EndIf
% \EndWhile
% \State \Comment{Return the best obtained configuration}
% \State $c_h, c_l, r$ = \Call{Opt}{$M_H$}
% % \EndProcedure
% \end{algorithmic}
% \end{small}
% \end{algorithm}

==> deprecated/experiment.tex <==
\section{Experiment Evaluation}
\label{sec:experiments}

In this section, we experimentally evaluate UDO on different workloads (TPC-C and TPC-H) and DBMSs (MySQL and Postgres). We also compare against different baseline methods highlighting different optimization (Quro, Dexter, PGTuner, MySQLTuner) and reinforcement learning (DDPG, SARSA) aspects of our system. 

\junxiong{Mention verions of Python 3}

Now, we briefly state our experimental setup. In Sec 10.1, we introduce baselines that focus on different optimization and RL aspects of the universal optimization problem. Following that, we show that for both TPC-C and TPC-H, and both Postgres and MySQL UDO outperforms all the baselines. We conclude this section by analysing effects of different reordering algorithms (Greedy and ILP) and delays on UDO's performance.

\noindent\textbf{Experimental Setup.} We use a server with 2 Intel Xeon Gold 5218 2.3 GHz CPUs having 32 physical cores and 384~GB of RAM for our experiments. To demonstrate that UDO can incorporate various DBMSs, we test UDO for MySQL(v5.7.29) and Postgres(v10.15). We  implement UDO in Python~3, using OpenAI gym~\footnote{https://gym.openai.com/}.

\subsection{Baselines}
We consider two types of baselines: traditional optimization methods and reinforcement learning based methods. 

\subsubsection{Traditional optimization methods.} For transaction reorder, we use \textit{Quro}~\cite{Yan2016} as the baseline. After extracting transaction units from each transaction, Quro invokes transactions and measures the running time of each unit for the given workload. Following that, it calculates the variance of the execution time for each transaction unit considered as conflict index, and solve the reorder unit problem by formalizing it as an integer programming problem. 
For index recommendation, we consider Dexter~\cite{dexter} as a baseline, which analyzes Postgres log files and generates indexes based on query frequencies. 
For system parameters, two well-known tuning tools, \textit{MySQLTuner}\footnote{https://github.com/major/MySQLTuner-perl} and \textit{PGTuner}~\footnote{https://github.com/jfcoz/postgresqltuner}, are utilized as baselines. 

\subsubsection{Reinforcement learning methods.}
We compare UDO with several Reinforcement Learning (RL)-based algorithms. All RL baselines adopts the 1-level UDO MDP formulations, and do not separate heavy parameters from light parameters. DDPG (Deep Deterministic Policy Gradient)~\cite{Lillicrap2016} is an actor-critic architecture based deep RL algorithm. SARSA~\cite{rummery1994line} is an on-policy learning algorithm. We implemented \textit{DDPG} and \textit{SARSA} algorithm for UDO using keras-RL~\footnote{\url{https://github.com/keras-rl/keras-rl}}. We also compare with RL algorithms for a sub-space problem, e.g., index recommendation. In particular, we use NoDBA~\cite{Sharma2018} as a baseline, which trains a deep neural network to predict the correct index configurations.

Also, we compare against \textit{simplified UDO} algorithm that applies the same delayed-HOO algorithm as UDO, but neither separates heavy and light parameters nor exploits delayed evaluations. 

% \begin{itemize}
%     \item Traditional optimizer.
%     \item Machine learning based optimizer.
% \end{itemize}

% \begin{itemize}
%     \item Quro \cite{Yan2016} decomposes the workload into several units, measures the runtime of each unit for the given workload and calculates the variance of the execution time of each operation as the conflict indexes and solve the reorder unit problem by minimizing the objective function given the operation unit constraint. 
%     \item NoDBA, utilizes the deep reinforcement learning to train a neural network to predict the correct index configurations.
%     \item MySQLTuner, is an auto turning tools for MySQL and it adjust the MySQL parameters to increase performance and stability.
%     \item DDPG, 
%     \item SARS
%     \item PGTuner
%     \item Dexter
% \end{itemize}

% (but not using the UDO-specific amortization of configuration change cost).

% Also, we compare against a simplified UDO version that does not separate heavy from light parameters and does not exploit delayed evaluations either. Finally, we compare against more traditional tuning tools and combine their solution for different classes of parameters. Namely, we set system parameters for Postgres (we use Postgres~10.15) via PGTuner ~\footnote{https://github.com/jfcoz/postgresqltuner} and select indexes via Dexter~\cite{dexter}. For MySQL (MySQL~5.7.29), we set system parameters via MySQLTuner \footnote{https://github.com/major/MySQLTuner-perl}, using indexes recommended by Dexter for Postgres which turned out to be equivalent to indexes recommended by another baseline we tried directly on MySQL, NoDBA~\cite{sharma2018case}, for the following experiments. We use Quro~\cite{yan2016leveraging} as baseline for optimizing query order in transactions.
\input{fig/tpcc_performance}
\subsection{TPC-C workload}
The TPC-C workload is an on-line transaction processing benchmark, which consists of 9 tables and 5 different type concurrent transactions. It has become the industry standard to evaluate the performance of OLTP systems. We initialize a database with 10 warehouses and set the number of concurrent request to 32 in the following experiment. For UDO, we set the horizon of heavy parameter MDP to 4 (implying the maximal number of indexes to select is 4) and the horizon of light parameter MDP to 8 (implying the maximal modification of the default configuration is 8). For other reinforcement learning baselines (the simplified UDO, DDPG and SARSA), they employ the 1-Level MDP which does not separate heavy from light parameters and does not exploit delayed evaluations either. We set the horizon of that 1-Level MDP to 12 indicating the maximal modifications of default configuration is 12. We warm up our system around ten minutes and transaction statistics are collected after the warm-up period. We test all baselines 4 hours and obverse the performance change for different baselines. Notice that, after keep running transaction in a long period, the throughput of DBMS may decrease because data volume gets larger. To keep a stable performance, for 1-Level MDP, we reset the database to the initial state after every episode. And for 2-Level MDP, we reset the database to the initial state after every delay \junxiong{every delay maybe not confused here}. We only build primary key indexes on those two DBMS for TPC-C benchmark.

\junxiong{Mention the number of delay in experiment setup}

\subsubsection{MySQL}
For mysql, the action space include 71 actions for indexes, 16 actions for transaction template reorder and 25 actions for system parameter. The state space is $2^{71} \times (7! \times 7! \times 5!) \times 1280 \approx 9.2 e^{33}$. The experiment results are shown in \ref{fig:mysql_tpcc}

Compared to other learning-based baselines and traditional baselines, UDO achieves significantly faster iterations due to delayed evaluations and cost-based planning.

\subsubsection{Postgres}
For postgres, the action space include 71 actions for indexes, 16 actions for transaction template reorder and 38 actions for system parameter, 125 actions in total. The state space is $2^{71} \times (7! \times 7! \times 5!) \times 230400 \approx 1.6 e^{36}$.

\input{fig/tpch_performance}
\subsection{TPC-H workload}
The TPC-H workload is an on-line analytical benchmark. It consists of 8 tables and 22 queries. We create a TPC-H database with scale factor 1. We set the horizon of heavy parameter MDP to 4 (implying the maximal number of indexes to select is 4) and the horizon of light parameter MDP to 5 representing the maximal changes of light system parameters. However, for the 1-Level MDP, the horizon is set to 9.

\subsubsection{Mysql}
For mysql, the action space include 99 actions for indexes and 25 actions for system parameter.


\subsubsection{Postgres}
For mysql, the action space include 99 actions for indexes and 38 actions for system parameter.



\subsection{Analysis of optimization overhead}

% micro episode	index time baseline(s)	index time delay(s)	total time baseline(s)	total time delay(s)
\input{fig/overhead_tpcc}
\subsubsection{TPC-C optimization overhead of different RL algorithms}

\input{fig/overhead_tpch}
\subsubsection{TPC-H optimization overhead of different RL algorithms}

\input{fig/reorder}
\subsection{Analysis of different reorder algorithm}

\input{fig/delays}
\subsection{Analysis of different delay}

\input{fig/single}
\subsection{Analysis of different UDO variant}

%\immanuel{For the last figure (delays), the axis labels make no sense to me. Junxiong, can you check this figure again?}

\immanuel{In general: many of the figures in this section miss legends and the axis labels lack units. Please add! Also, please add a little description (catchwords are fin) about each figure, stating the whole setup (which benchmark, which system).}

==> deprecated/formalization.tex <==
\section{Formal Model}
\label{sec:model}

% We formalize UDO (universal database optimization) as an episode MDP. The state space $S=S_h\times S_l$ integrates two sub-spaces, light parameters and heavy parameters. Heavy parameters represent those parameters which are expensive to change, while light configurations include those parameters which are easy to switch. We represent $S_h$ and $S_l$ as partial functions, representing a partially specified configuration. More precisely, $S_h:H\mapsto\mathbb{R}$ is a function mapping a set $H$ of system heavy parameters to admissible values (assumed numerical), and $S_l:L\mapsto\mathbb{R}$ a function mapping a set $L$ of light parameters to admissible values.

% \begin{definition}
% The \textbf{universal database optimization} (UDO) is defined as a MDP problem, where the state space $S=S_h \times S_l$ integrates two sub-spaces, $S_h$ for heavy parameters that are expensive to change and $S_l$ for light parameters that are easy to switch. 
% \end{definition}

\begin{definition}
\textbf{Range of a parameter} is defined as admissible values of a given parameter, which is predetermined by users or underlying databases.
\end{definition}

\begin{example}
The range of a index parameter is $\{0, 1\}$, indicating whether the  corresponding index is created or not. The range of a system parameter is a array including its validate values. For example, the validate values of random\_page\_cost in Postgres is $[0, 1.79769 e^{308}]$, UDO can take a subset $\{0, 4, 10, 100, 10^3, 10^4\}$ as its range. For the transaction unit reorder, The range of a query template unit is $\{0, 1, \cdots, N-1\}$, where $N$ is the number of total reorder unit. 
\end{example}

\begin{definition}
A \textbf{parameter vector} is a collection of all possible tuning parameters.
% \deba{A vector cannot be a space. A space is a set of vectors or in this case a tuple of ranges of parameters. Present definition represents a parameter list/set.}
\end{definition}

\begin{example}
\{random\_page\_cost, seq\_page\_cost, index a, index b, enable\_mergejoin\} can be a parameter vector.
\end{example}

% \junxiong{change to the vector representation}

\begin{definition}
% Given a parameter vector $P$, a \textbf{configuration} $c$ is a vector in which each element is constructed by taking one value in the range of each parameter in the space $P$,
Given a parameter vector $P$, a \textbf{configuration} $c$ is a vector and each element in $c$ is constructed by taking one value in the range of the corresponding parameter in vector $P$, i.e., $c[i] \in \text{Range}(P[i]), \forall i \in \{0, 1 \cdots, P.len\}$.
% that parameter vector
% \junxiong{I don't know how to write it in math formula, $[\text{Range}(p) \text{ for } p \in P]$? or $Range(P)$ }
% A \textbf{configuration} is a vector and each element in this vector represents a value in its range of a specific parameter.  
% A \textbf{configuration} is defined as an instance of given parameters. 
% We represent $S_p$, $S_i$, and $S_o$ as partial functions, representing a partially specified configuration. More precisely, it is $S_p:P\mapsto\mathbb{R}$ a function mapping a set $P$ of system parameters to admissible values (assumed numerical). Function $S_i:I\mapsto\mathbb{B}$ maps index candidates to Boolean values, indicating whether the corresponding index is created or not. Finally, function $S_o:Q\mapsto\mathbb{N}$ maps queries within transaction templates to positions at which they are executed.
% \immanuel{Please make that more precise by adding a mathematical formula here}
\end{definition}


\begin{definition}
% A \textbf{configuration space} $C$ w.r.t. a given parameter vector $P$ is defined as all possible configurations $c$ constructed from the given parameter vector, i.e., $\{c | c[i] \in \text{Range}(P[i]), \forall i \in \{0, 1 \cdots, P.len\}\}$.
A \textbf{configuration space} $C$ is jointly defined by a parameter vector $P$ and ranges of parameters includes all possible configurations $c$, i.e., $\{c | c[i] \in \text{Range}(P[i]), \forall i \in \{0, 1 \cdots, P.len\}\}$.
\end{definition}
% \deba{A configuration space is jointly defined by the `parameter list' and `ranges of parameters'.}
% \immanuel{what does validate mean here?}
% \immanuel{please add formula}

\begin{example}
For the parameter vector \{random\_page\_cost, index a, index b, enable\_mergejoin\}, if $Range(random\_page\_cost) = \{0, 4, 10, 100\}$, a configuration can be $[4, 0, 1, 0]$. The cardinality of the configuration space is $4 \times 2 \times 2 \times 2 = 32$
\end{example}

\begin{definition}
\textbf{Performance function} $f:C\mapsto\mathbb{R}$ is a function mapping a specific configuration in a configuration space $C$ to its performance for the given workload $W$. For OLTP workloads, performance of a configuration is defined as the throughput (i.e., committed transactions per second) of that configuration. For OLAP workloads, performance of a configuration is defined as the
negative of the execution time of the given workload with that configuration. 
\end{definition}

\begin{definition}
The \textbf{universal database optimization problem} is defined as given a workload $W$, a configuration space $C$ 
% \deba{shouldn't it be configuration space $C$?} and a time budget $T$ 
% \deba{Time budget is an artifact of our solution process but not the optimisation problem itself}
% \immanuel{Timeout would apply to all iterative algorithms but ok with leaving it out}
, the task is to find a configuration $c^{\star} \in C$ to maximize the performance function $f$, i.e., $c^{\star} \triangleq \argmax_{c \in C} f(c|W)$. In practice, we assume UDO is given a time budget $T$ and the goal is to find a best configuration within this time budget.
%  w.r.t. given tuning parameter space
% \deba{\begin{equation*}
%     c^* \triangleq \argmax_{c \in C} f(c|W).
% \end{equation*}}
\end{definition}

\begin{definition}
The \textbf{episodic MDP for naive UDO} is represented by $(\mathcal{S}, \mathcal{A}, \mathcal{T}, H, R)$, where $\mathcal{S}$ is the state space, defined as the configuration space $C$, $\mathcal{A}$ is the action space, defined as all validate changes of configurations (i.e., the value of changed parameter is in its range), $\mathcal{T}: \mathcal{S} \times \mathcal{A} \mapsto \mathcal{S}$ is the transition from the current state and a selected action to the next state, $H$ is the horizon indicating the number of maximal steps, $R: \mathcal{S} \times \mathcal{A} \mapsto \mathbb{R}$ is the reward function, representing the performance improvement from state $s_1$ and taking action $a$ to state $s_2$, i.e., $f(s_2) - f(s_1)$. The goal is to find a policy which maximizes the accumulated reward.
% $H$ is the number of maximal steps
% and $N$ is the stimulated maximal episode determined by the time budget $T$. 
\end{definition}
% \deba{Why specifying `simplified' here? Rather this MDP formulation is natural after the previous equation.}

% The universal database optimization problem can be solved using reinforcement learning models by formalizing as an episodic MDP problem, represented by $(\mathcal{S}, \mathcal{A}, P, N, H, R)$, where $\mathcal{S}$ is the state space, defined as the configuration space $C$, $\mathcal{A}$ is the action space, defined as all validate changes of configurations, $P: \mathcal{S} \times \mathcal{A} \mapsto \mathcal{S}$ is the transition from the current state and a selected action to the next state, $R: \mathcal{S} \times \mathcal{A} \mapsto \mathbb{R}$ is the reward function, representing the performance improvement from state $s_1$ and taking action $a$ to state $s_2$, i.e., $f(s_2) - f(s_1)$, $H$ is the number of maximal steps, and $N$ is the stimulated maximal episode. The goal is to find a policy which maximizes the accumulated reward.

%  \immanuel{I understood we currently use a different mechanism for light parameters" I believe that the reward is only calculated after all light parameters are specified? The performance improvements were only measured for heavy parameters IMO?}

\begin{example}
Given the TPC-C workload, and a parameter vector [index a, index b, seq\_page\_cost, random\_page\_cost, enable\_bitmapscan, enable\_mergejoin], if the range of seq\_page\_cost and random\_page\_cost is $[4, 10, 100]$ and the range of enable\_bitmapscan, enable\_mergejoin is $[0, 1]$, the validate configuration space w.r.t. that parameter vector includes 144 configurations. Thus the state space $\mathcal{S}$ has 144 states, and the action space $\mathcal{A}$ has $14$ actions. One state $s$ should represent a configuration $[1, 0, 100, 4, 1, 1]$. At this state $s$, one action $a_1$ should be creating the index $b$ which transition to anther state $s^{\prime}$ representing a configuration $[1, 1, 100, 4, 1, 1]$. Thus the transition matrix $P$ should include the transition from $s$ and $a_1$ to $s^{\prime}$. If we suppose $f(s) = 6000, f(s^{\prime}) = 7000$, the $(s, a_1)$ entry in the reward matrix $R$ should be 1000. 
% where index a is CUSTOMER(C\_D\_ID, C\_LASTNAME), index b: NEW\_ORDER(NO\_D\_ID, NO\_O\_ID), seq\_page\_cost, random\_page\_cost, enable\_bitmapscan, enable\_mergejoin. 
% have three discretized values 4, 10 and 100, and enable\_bitmapscan, enable\_mergejoin have two discretized values 0 and 1. The validate configuration space w.r.t. those parameters includes 144 configurations.
% One state $s$ should include the configuration (index a, seq\_page\_cost=100, enable\_bitmapscan=1) where we omit the default system parameters (i.e., since random\_page\_cost, enable\_mergejoin. uses its default value, we do not include them in the state $s$ explicitly). At state $s$, one action $a_1$ should be creating the index $b$ which transition to anther state $s^{\prime}$ (index a, index b, seq\_page\_cost=100, enable\_bitmapscan=1). Thus the transition matrix $P$ should include the transition from $s$ and $a_1$ to $s^{\prime}$. If we suppose $f(s) = 6000, f(s^{\prime}) = 7000$, the reward for $(s, a_1)$ should be 1000. 
% \junxiong{should we describe the reward scale here?}
\end{example}

% \begin{definition}
% We represent $F_h$ and $F_l$ as partial functions, representing the performance of a partially specified configuration. More precisely, $F_h:S_h\mapsto\mathbb{R}$ is a function mapping a specific heavy configuration in $S_h$ to an admissible value (assumed numerical), and $F_l:S_l\mapsto\mathbb{R}$ is a function mapping a specific light in $S_l$ to an admissible value.  
% \end{definition}


\begin{definition}
We decompose a parameter vector $P$ into $P_h \times P_l$, where $P_h$ is for \textbf{heavy parameters} that are expensive to change and $P_l$ is for \textbf{light parameters} that are easy to switch. Configurations generated from the $P_h$ are \textbf{heavy configurations} $C_h$ while configurations generated from the $P_l$ are \textbf{light configurations} $C_l$. 
\end{definition}

\begin{example}
For OLTP workloads, indexing decisions ($P_i$) and materialized view ($P_v$) can be considered as heavy parameter. System parameters ($P_p$) and in-transaction query ordering decisions ($P_o$) belong to light parameters.
\end{example}


\begin{example}
For OLAP workloads, indexing decisions ($P_i$) and materialized view ($P_v$) can be considered as the heavy parameter while system parameters ($P_p$) and join orders ($P_j$) are light parameters.
\end{example}

% Actions correspond to changes to configurations, including heavy configurations and light configurations. 

% \begin{example}
% Actions may include changing a tuning parameter value, creating or dropping an index, or swapping the order of two queries within the same transaction template. 
% \end{example}

After separating the configuration space, the ultimate goal becomes finding a best combination of heavy configuration and light configuration maximing the performance function $f$.

% An episode MDP problem is given by a tuple $(\mathcal{S}, \mathcal{A}, H, N, M)$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $H$ is the number of horizon, $N$ is the number of episode. Each step


% We iteratively build the global search tree using the Monte Carlo simulation (i.e., we traverse the search tree from root and pick up one action each step), build the parameters that we choosed. Frequently switching heavy parameters has large overhead.

% \immanuel{The paragraph below already describes a way to solve the problem - this section should be only about describing the problem, please remove}

% we propose a \textbf{two level episodic reinforcement learning} algorithm, presented in Algorithm ~\ref{alg:two_level}. 
UDO learns the optimal configurations using a two level approach. 
% At the top level, UDO uses a episodic MDP model to learn best heavy configurations. 
At the top level, UDO models the learning of heavy configurations as an episodic MDP under the delayed feedback. At bottom level, UDO constructs an episodic MDP model for each heavy configuration to learn the best light configuration under a specific heavy configuration. 

% Our algorithm integrate two level episodic MDP models including a delay episodic MDP model for heavy configurations and a non delay episodic MDP model for light configurations. 

% \immanuel{there is no such thing as a delayed MDP - this is a property of the algorithm!}
% \deba{From this paragraph, even from the point we separated the heavy and light parameters, we are getting into our approach/solution. The problem inherently does not require this. We should clarify that.}

% \junxiong{change the delay}

\begin{definition}
The \textbf{episodic MDP under delayed feedback for heavy parameters} is given by a tuple $\mdp_h \triangleq (\mathcal{S}_h, \mathcal{A}_h, \mathcal{T}_h, R_h, H_h)$. $\mathcal{S}_h$ is the is the state space for heavy configurations. $\mathcal{A}_h$ is the action space representing changes of heavy configurations. $\mathcal{T}_h: \mathcal{S}_h \times \mathcal{A}_h \mapsto \mathcal{S}$ is the transition from state $s_1 \in \mathcal{S}_h$ representing a heavy configuration and a selected action $a_1 \in \mathcal{A}_h$ (i.e., change value of one heavy parameter) to the next state $s_2 \in \mathcal{S}_h$ representing another heavy configuration. $R_h: \mathcal{S}_h \times \mathcal{A}_h \mapsto \mathbb{R}$ is the reward function, representing the performance improvement from a state $s_1$ and an action $a_1$ to the next state $s_2$, i.e., $r(s_1, a_1) = \max_{s_l \in S_l} f(s_l, s_2) - \max_{s_l \in S_l} f(s_l, s_1) \text{ where } s_2 = \mathcal{T}_h(s_1, a_1)$ where $S_l$ is the state space of light configurations. $H_h$ is the horizon indicating the number of maximal steps for heavy parameters.
% \junxiong{Should we also add the initial state $s_0$ and the V-value of s, and Q value of (s, a)}

% $s_l^1, s_l^2$ representing the best light configuration retrieved from the bottom reinforcement learning model parameterized by heavy configuration state $s_1$ and $s_2$ respectively. 
% $N_2$ is the number of the simulation episodes and $d$ is the maximal tolerance of delay time.
\end{definition}

% The \textbf{delay episodic MDP} is given by a tuple $(\mathcal{S}_2, \mathcal{A}_2, P_2, H_2, N_2, d)$. $\mathcal{S}_2$ is the state space  including all validate heavy configurations. $\mathcal{A}_2$ is the action space representing changes of heavy configurations. $P_2: \mathcal{S}_2 \times \mathcal{A}_2 \mapsto \mathcal{S}$ is the transition from state $s_1 \in \mathcal{S}_2$ representing a heavy configuration and a selected action $a_1 \in \mathcal{A}_2$ (i.e., change value of one heavy parameter) to the next state $s_2 \in \mathcal{S}_2$ representing another heavy configuration. $R_2: \mathcal{S}_2 \times \mathcal{A}_2 \mapsto \mathbb{R}$ is the reward function, representing the performance improvement from state $s_1$ and $a_1$ to $s_2$, i.e., $f(s_2 \circ s_l^2) - f(s_1 \circ s_l^1)$ where $s_l^1, s_l^2$ representing the best light configuration retrieved from the bottom reinforcement learning model parameterized by heavy configuration state $s_1$ and $s_2$ respectively.
% % representing the best light configuration retrieved from the bottom reinforcement learning model parameterized by heavy configuration state $s_2$ and $s_l^1$ is the best light configuration returned from the bottom reinforcement learning model parameterized by heavy configuration state $s_1$ 
% $H_2$ is the number of maximal modification allowed for heavy parameters, $N_2$ is the number of the simulation episodes for heavy parameters, $d$ is the maximal tolerance of delay time.

% \immanuel{Please distinguish between properties of the algorithm and of the MDP. $N$ and $d$ should be tuning parameters of the algorithm IMO.}

% $H_2$ is the number of horizon, $N_2$ is the number of episode and $d$ is the maximal tolerance of delay time. 

% For UDO, $\mathcal{S}_2$ is the space of heavy parameters including all valid heavy configurations, $\mathcal{A}_2$ is the action space representing a specific change of heavy configurations, $H_2$ is the number of maximal modifications to the default heavy configuration and $N_2$ is the number of simulated episodes for a selected heavy configuration. The reward is the maximal performance improvement returned by its reinforcement learning model for light parameters.

% The \textbf{delay episodic MDP} is given by a tuple $(\mathcal{S}_2, \mathcal{A}_2, H_2, N_2, d)$, where $\mathcal{S}_2$ is the state space, $\mathcal{A}_2$ is the action space, $H_2$ is the number of horizon, $N_2$ is the number of episode and $d$ is the maximal tolerance of delay time. For UDO, $\mathcal{S}_2$ is the space of heavy parameters including all valid heavy configurations, $\mathcal{A}_2$ is the action space representing a specific change of heavy configurations, $H_2$ is the number of maximal modifications to the default heavy configuration and $N_2$ is the number of simulated episodes for a selected heavy configuration. The reward is the maximal performance improvement returned by its reinforcement learning model for light parameters.

% For OLAP workload, the scaled query time is the reward. For OLTP workload, the scaled throughput is the reward. The whole procedure is that UDO starts from episode $1$ to $N_1$, at each episode, UDO starts from the default configuration (i.e., start state) and iteratively modifies the current configuration from the step $1$ to $H_1$ based on the statistics of actions, evaluates the final configuration to obtain the reward and update the statistics of selected actions. 

\begin{example}
Given the heavy parameter vector [index a, index b, index c, index d], for the episodic MDP for heavy parameters, the cardinality of its state space $\mathcal{S}_h$ and action space $\mathcal{A}_h$ is 16 and 8 respectively. $\mathcal{T}_h$ should include a transition from a state $s$ representing a configuration $[0, 0, 1, 1]$, and an action $a_1$ creating index b to another state $s^{\prime}$ representing another heavy configuration $[0, 1, 1, 1]$. Supposing the largest performance function value for the state $s$ is 3000 and for the state $s'$ is 4000, we have $R(s, a) = 1000$.
\end{example}


\begin{definition}
The \textbf{episodic MDP for light parameters}, is proposed to learn a best light configuration under a specific heavy configuration, represented by $\mdp_l(s_h) \triangleq (\mathcal{S}_l, \mathcal{A}_l, \mathcal{T}_l, H_l, R_l)$ where $\mathcal{S}_l$ is the state space representing light configuration space $P_l$ parameterized by the heavy configuration state $s_h$. $\mathcal{A}_l$ is the action space representing validate changes of light configurations. $\mathcal{T}_l: \mathcal{S}_l \times \mathcal{A}_l \mapsto \mathcal{S}_l$ is the transition from a light configuration state $s_l \in \mathcal{S}_l$ and a selected action $a_1 \in \mathcal{A}_l$ (i.e., change value of one parameter) to the next state $s_2 \in \mathcal{S}_l$. $H_l$ is the horizon defining the number of maximal modifications allowed for light parameters. $s_h$ is the given heavy state. $R_l:\mathcal{S}_l \times \mathcal{A}_l \mapsto \mathbb{R}$ is the reward function, representing the performance improvement from a state $s_1$ and an action $a_1$ to the next state $s_2$, i.e., $r(s_1, a_1) = f(s_2, s_h) - f(s_1, s_h) \text{ where } s_2 = \mathcal{T}_l(s_1, a_1)$.
% and $N_h$ is the number of the simulation episode depend on the time budget $T$
\end{definition}

% \deba{The symbol $\circ$ is typically used for composition of functions. we can use simply $(s_2, s_h)$ here and $\times$ for Cartesian product. }

% \immanuel{Please add more details in this definition, e.g. mathematically define, via a formula, the state resulting from applying an action to another state}


% The \textbf{non delay episode MDP} is proposed to learn a best light configuration under a specific heavy configuration. A delay episodic MDP is represent by $(\mathcal{S}_1, \mathcal{A}_1, P_1, H_1, N_1, R_1, s_h)$ where $\mathcal{S}_1$ is the state space including all validate light configurations, $\mathcal{A}_1$ is the action space representing all validate changes of light configurations, $s_h$ is a state of the delay MDP model at top level representing a heavy configuration, $P_1: \mathcal{S}_1 \times \mathcal{A}_1 \mapsto \mathcal{S}$ is the transition from the current light configuration state $s_1 \in \mathcal{S}_1$ and a selected action $a_1 \in \mathcal{A}_1$ (i.e., change value of one parameter) to the next state $s_2 \in \mathcal{S}_1$ representing the new light configuration, $R_1: \mathcal{S}_1 \times \mathcal{A}_1 \mapsto \mathbb{R}$ is the reward function, representing the performance improvement from state $s_1$ and $a_1$ to $s_2$, i.e., $f(s_2 \circ s_h) - f(s_1 \circ s_h)$, $H_1$ is the number of maximal modification allowed for light parameters and $N_1$ is the number of the simulation episode. 



% For UDO, $\mathcal{S}_1$ is the space of light parameters including all valid light configurations, $\mathcal{A}_1$ is the action space representing a specific change of light configurations, $H_1$ is the number of maximal modifications to the default light configuration and $N_1$ is the number of simulated episodes. The reward is the performance change compared with the default configuration. For OLAP workload, the scaled query time is the reward. For OLTP workload, the scaled throughput is the reward. The whole procedure is that UDO starts from episode $1$ to $N_1$, at each episode, UDO starts from the default configuration (i.e., start state) and iteratively modifies the current configuration from the step $1$ to $H_1$ based on the statistics of actions, evaluates the final configuration to obtain the reward and update the statistics of selected actions. 

\begin{example}
At the top level, UDO selects a heavy configuration $[1, 1, 0]$ (i.e., building index A and B, not C), and builds a reinforcement learning model for this heavy configuration. The light parameter vector is [random\_page\_cost, seq\_page\_cost, enable\_bitmapscan, enable\_mergejoin], if the range of seq\_page\_cost and random\_page\_cost is $[4, 10, 100]$ and the range of enable\_bitmapscan, enable\_mergejoin is $[0, 1]$, the validate light configuration space has cardinality 36. The state space $\mathcal{S}_l$ has 36 states, and the action space $\mathcal{A}_l$ has $10$ actions. $\mathcal{T}_l$ should include a transition from a state $s$ representing a configuration $[4, 4, 1, 1]$, and an action $a_1$ setting the random\_page\_cost to $100$ to another state $s^{\prime}$ representing a configuration $[100, 4, 1, 1]$. Supposing $f(s) = 6000$ and $f(s^{\prime}) = 7000$, then we have $R(s, a_1) = 1000$.
% At the top level, UDO selects the index A, B and C as heavy configurations (state $[1, 1, 1, 0]$) and builds a reinforcement learning model for this heavy configuration. 
% The available light parameters are random\_page\_cost (4, 10, 100), seq\_page\_cost (4, 10, 100), enable\_bitmapscan (0, 1), enable\_mergejoin (0, 1) and force\_parallel\_mode (0, 1). If we set $N_1 = 10, H_1 = 5$, UDO simulates this reinforcement learning model 10x, and the maximal selected actions in each episode is five. The reinforcement learning model should try 10 episodes. During the first episode, the agent starts from the initial state, may choose the action, setting random\_page\_cost to 10, reaching to the state (random\_page\_cost = 10). Then the agent chooses another action, setting force\_parallel\_mode to 0, reaching to the state (random\_page\_cost = 10, force\_parallel\_mode = 0). The agent keeps picking up actions until reaching the the horizon $H_1 = 5$. If the agent reach to the final state (random\_page\_cost = 10, force\_parallel\_mode = 0, enable\_mergejoin = 1, enable\_bitmapscan = 0, seq\_page\_cost = 100), UDO switches to this configuration , evaluates the workload and updates the model using the performance information. UDO repeats this procedure until finishing ten episodes.  
\end{example}

% The heavy configuration candidates may be index A, B, C, D, E and F. If we set the $H_2$ to three, the maximal number of indices picked by UDO is three. During one episode, the agent starts from an empty index set, may picking up indices A at step one, B at step two and C at step three. Then the agent build three light MDP models parameterized by heavy configuration (A), (A, B) and (A, B, C). Once finishing the simulation of those three underlying MDP models, The agent retrieves three best light configurations for heavy configurations (A), (A, B) and (A, B, C). Supposing the largest performance function value for configuration (A) is 3000, for configuration (A, B) is 4000, and for configuration (A, B, C) is 6000. The reward of the state (A) and action creating index B is 1000, and the reward of the state (A, B) and action creating index C is 2000.


% A delay episodic MDP is given by a tuple $(\mathcal{S}_1, \mathcal{A}_1, H_1, N_1, d)$, where $\mathcal{S}_1$ is the state space, $\mathcal{A}_1$ is the action space, $H_1$ is the number of horizon, $N_1$ is the number of episode and $d$ is the maximal tolerance of delay time. A non-delay episode MDP model is represent by $(\mathcal{S}_2, \mathcal{A}_2, H_2, N_2)$ where $\mathcal{S}_2$ is the state space, $\mathcal{A}_2$ is the action space, $H_2$ is the number of horizon and $N_2$ is the number of episode.
% % UDO adopts the delay MDP to learn the heavy configurations and adopts the non delay MDP to learn light parameters. 
% For UDO, $\mathcal{S}_1$ is the state space of heavy parameters, $\mathcal{A}_1$ is the action space of heavy parameters, $N_1$ is the number of simulated episodes depends on the tuning time, $H_1$ is the maximal modification allowed for heavy parameters (e.g., if the heavy parameters represent indices, $H_1$ is the number of selected indices). $\mathcal{S}_2$ is the space of light parameters, $\mathcal{A}_2$ is the action space of light parameters, $H_2$ is the number of maximal modification for light parameters and $N_2$ is the number of simulated episodes. Then, the light parameter $N_2$ is the number of simulation for each selected heavy parameter.

% \immanuel{Please remove any algorithms from the formal model section - the goal here is only to introduce the problem, not the solution.}

==> deprecated/version2/learning.tex <==
\section{Reinforcement Learning}\label{sec:rlalgs}
% UDO uses RL algorithms to find optimal settings for heavy and light parameters. The goal of separating heavy from light parameters is to enable us to use different RL algorithms for both types of parameters. We will vary the RL algorithms used in our experiments. Next, we give a quick overview of the different RL algorithms used by our main version. We refer to an extended technical report for details.

UDO uses Monte Carlo Tree Search (MCTS) \citep{Coquelin2007a}, which is a family of RL algorithms, to solve the light and heavy parameter UDO MDPs in order to obtain optimal light and heavy configurations.
We propose two layers of contributions in using RL algorithms. At first, we propose to use delayed bandit algorithm $\alg$ in MCTS framework to formulate \textit{delayed-MCTS}. We show that $\alg$ can incorporate different algorithms, such as delayed-UCB-V\footnote{We propose delayed-UCB-V by combining the delayed feedback management schematic of~\cite{Joulani2013a} and UCB-V~\citep{ucbv}.} and delayed-EXP3~\citep{li2019bandit}. 
Following that, we incorporate delayed-MCTS with delay $0$ and $\tau > 0$ for solving the light and heavy parameter UDO MDPs, respectively. This framework allows us to evaluate the light parameter configurations at every step while delaying evaluation of heavy parameter configurations by $\tau$. This allows UDO to obtain speed-up in comparison to the 1-level UDO MDP as shown in Section~\ref{sec:experiments}.

\begin{algorithm}[t!]
\caption{RL: Monte Carlo Tree Search with Delayed Feedback (Delayed-MCTS)}
\label{alg:delay_mcts}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} Delayed bandit algorithm $\alg$, configuration space $C = C_H$ (for heavy parameters) and $c_H \times C_L$ (for light parameters), current state $c_t$
\State \textbf{Output:} Final parameter configuration
\Function{RL.Select}{$\alg, C, c_t$}
    \If{$c_t$ is not a terminal state}
        \State Obtain $a_t \leftarrow$ \Call{$\alg$.SelectionPolicy}{$c_{t}, \tau, C$}
        \State Sample $c_{t+1} \sim \mathcal{T}(c_{t}, a_t)$
        \State \Return Configuration $c_{t+1}$
        %\State $AList \gets AList \circ a_t$
        \Else \Return Configuration $c_{t}$ 
    \EndIf
\EndFunction
\vspace{0.25cm}
\State \textbf{Input:} Updated evaluation $E$, delayed bandit algorithm $\alg$
\Procedure{RL.Update}{$\alg, E$}
    \State \Comment{Obtain evaluated $c,a,r$ tuples till time $T$}
    \State $\{c_i, a_i, r_i\}_{i=0}^t \gets E$
    \State \Call{$\alg$.UpdatePolicy}{$\{c_i, a_i, r_i\}_{i=0}^t$}
\EndProcedure
% \EndFunction
\vspace{0.25cm}
\State \textbf{Input:} Delayed bandit algorithm $\alg$, configuration space $C$, current state $c_t$, time budget $T$
\State \textbf{Output:} Final parameter configuration
\Function{RL.Optimize}{$\alg, C, c_0, T$}
\State Initialize $Stat \gets \emptyset$
\For{$t=1, \ldots, T$}
\State $c_{t+1}, a_t \gets$ \Call{RL.Select}{$\alg, C, c_t$}
\State Evaluate the new configuration $r_t \gets$ \Call{B.Evaluate}{$c_{t+1}$}
%\State \Comment{Append observed $c, a, r, c'$ tuple at timestamp $t$}
\State Update $Stat \gets Stat \circ \{c_t, a_t, c_{t+1}, r_t, t\}$
\State \Call{RL.Update}{$\alg, Stat$}
\EndFor
\State \Return Final parameter configuration $c_T$
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

In Algorithm~\ref{alg:delay_mcts}, we elaborate the schematic of delayed-MCTS. We refer to this module as \textproc{RL} that offers three functions. First one is the action selection function \textproc{RL.Select}. Following the selection policy of delayed bandit algorithm $\alg$, \textproc{RL.Select} first takes an action $a_t$ from current configuration $c_t$.
For example, in case of delayed-UCB-V, we choose the action $a_t$ leading to configuration $c_{t+1}$ such that
\begin{align}
    c_{t+1} \triangleq \argmax_c \hat{r}_c(t)+\sqrt{2.4 \hat{\sigma}_c^2(t) \frac{\log(v_{c_t})}{v_c}} + \frac{3 b \log(v_{c_t})}{v_c},\label{eq:delayeducbv}
\end{align}
Here, $v_{c_t}$ and $v_c$ are the number of visits to the parent configuration $c_t$ and child configuration $c$ respectively. The average reward obtained till time $t$ after considering delay $\tau$, i.e. $\hat{r}_c(t) = \sum_{i=\tau}^t r(c_{i-\tau})\mathbbm{1}(c_{i-\tau}=c)$.
Similarly, $\hat{\sigma}_c^2(t)$ is the empirical variance of reward obtained from configuration $c$ after considering the delay $\tau$.
For delayed-EXP3~\citep{li2019bandit}, we choose an action $a$ with probability
\[ a_t \sim \mathbb{P}(a|c=c_t) \propto \exp\left[\sum_{i=\tau}^t \frac{r_{i}(c_t, a) \mathbbm{1}(a_{i-\tau}=a)}{\mathbb{P}_{i-\tau}(a|c_t)} \right].\]
In delayed-EXP3, the probability of choosing an action $a$ from a given state $c$ varies exponentially with the total accumulated reward considering delay and inverse probability of visiting $(c_t, a)$.
The second one is \textproc{RL.Update} that obtains evaluation $E$ at time $t$ and update statistics of $\alg$. Each evaluation $E$ contains a set of tuples $\{c_i, a_i, r_i, c_{i+1}\}$ till present time $t$.
For example, in case of delayed-UCB-V, we update the number of visits to state-action pair $(c_t, a_t)$, present state $c_{t+1}$, and sample mean and variance of accumulated rewards ($\hat{\mu}(c_t, a_t)$ and $\hat{\sigma}^2(c_t, a_t)$).
In case of delayed-EXP3, it updates the weights defining probability $\mathbb{P}(a|c=c_t)$ of taking any action $a$ from state $c_t$.

The third function is \textproc{RL.Optimize}. \textproc{RL.Optimize} essentially incorporates a delayed bandit algorithm $\alg$ in the classical MCTS framework. Till the imposed timeout is exhausted, it iteratively obtains next actions and configurations using \textproc{RL.Select}, evaluate this configuration, and use the newly observed state-action-reward triplet to update the statistical log of $\alg$ using \textproc{RL.Update}.  

\begin{example}[Delayed-UCT]
A specific instance of Algorithm~\ref{alg:delay_mcts} is the delayed-UCT algorithm. We propose a variant of UCB-V~\citep{ucbv} with delayed feedback as the selection policy $\alg.$\textproc{Selection} \textproc{Policy} and RAVE (Rapid Action Value Estimation)~\citep{Gelly2007} as the update policy $\alg.$\textproc{UpdatePolicy} of delayed-UCT.
At each node, the delayed-UCB-V selection policy selects the child node $c$ (representing a configuration) that has highest upper confidence on its own reward (Eq.~\ref{eq:delayeducbv}). 
RAVE update policy assumes that the value of an action $a$ taken from the state $c$ is similar with respect to all states within the subtree of state $c$. 
This assumption fits our problem as the selection order of configurations does not influence the final state and accumulated reward (e.g., same actions with different selection order lead to a same final state).
Combining UCB-V and RAVE, the selection policy for a child configuration $c$ becomes 
$$c^* \triangleq \argmax_c \tilde{r}_c+\sqrt{2.4 \tilde{\sigma}_c^2 \frac{\log(v_p)}{v_c}} + \frac{3 b \log(v_p)}{v_c}.$$ 
Here, $v_p$ is the number of visits to the parent node $p$ of configuration $c$ at level $l$ of the Monte Carlo tree.
$\tilde{v}_c = \sum_{i=1}^{v_p} \mathbbm{1}_{i} (c)$ is the total number of times $c$ appears as a direct or indirect child of $p$ and $p$ appears at level $l$.
The average reward obtained by $c$ under aforementioned conditions is $\tilde{r}_c = \frac{1}{\tilde{v}_c} \sum_{i=1}^{v_p} \mathbbm{1}_{i} (c) f_i(c)$. $f_i(c)$ is the reward, i.e. the performance measure, obtained by configuration $c$ in $i$-th evaluation.
$\tilde{\sigma}_c^2 =  \frac{1}{\tilde{v}_c} \sum_{i=1}^{v_p} \mathbbm{1}_{i} (c) f_i^2(c) -\tilde{r}_c^2$ is the empirical variance of reward obtained by $c$ under the same conditions. 

We refer to this combined version of algorithm with delayed-UCB-V and RAVE as the \textit{delayed-UCT} algorithm. As per our knowledge, though UCT is well-studied, we are the first to propose delayed-UCT that accommodates delayed feedback in UCT framework.
\end{example}

If we substitute the evaluation step of Line 23 in Algorithm~\ref{alg:delay_mcts} with the evaluation step of Lines 12-14 in Algorithm~\ref{alg:twoLevelVar}, we retrive the iterative procedure of UDO. This indicates that the general framework of UDO (Line 7- 20) is actually an extended MCTS algorithm that operates of the configuration space of heavy parameters. Since the utility of only heavy parameter configurations are not explicitly accessible, UDO utilises another MCTS algorithm (\textproc{RL.Optimize}) to evaluate the adjacent light parameter configurations (as described in Algorithm~\ref{alg:evalVar}). This two level MCTS approach provides us a chance to use a bandit algorithm $\alg_H$ with delay $\tau$ for heavy parameters where evaluation is time consuming, and an algorithm $\alg_L$ with no delay where evaluation is cheaper but accuracy is sought. Faster convergence is important for $\alg_L$ as we call it to evaluate each of the heavy configuration evaluated by UDO. We also focus on higher accuracy for $\alg_L$ as the bias remaining in its solution propagates to the solutions obtained by the $\alg_H$ and can amplify inaccuracy.
In the next section, we show that this two level delayed-MCTS approach incurs asymptotically vanishing regret for UDO.

==> revision/meta_reviewer.tex <==
\noindent {\LARGE\bf{\em Dear VLDB Associate Editor and Reviewers:}}

We thank the reviewers and editor for their helpful feedback! We added various new baselines and experiments and improved the presentation. We believe the revised version addresses all points.

% We thank the reviewers and the associate editor for the very helpful feedback on our paper. 
% We addressed all of the concerns and included references to the revised text. In the following, we address each reviewer's comments.

%first provide our responses to the meta review, then 

% \subsection*{\huge Meta Review Details.}
% \vspace{2ex}

% {\bf M1. \review{Please improve the presentation and experiments, add better justification of the design and proposed techniques, and discuss related work in details.}}

==> revision/response.tex <==
\begin{multicols}{2}

\input{revision/meta_reviewer}

\input{revision/reviewer1}

\input{revision/reviewer2}

\input{revision/reviewer3}

\end{multicols}

==> revision/reviewer1.tex <==
\begin{center}
\line(1,0){240}
\end{center}

\subsection*{\huge Review 1 Details} 

{\bf \review{
D1. Definition 2.4: I am a bit confused on the definition of f. Shouldn't this function depend on the benchmark as well as the configuration?
 }}

We have simplified the model in the revision. As outlined in Section~\ref{sec:model}, $f$ represents performance according to a specific metric for a specific workload. Hence, $f$ itself integrates the choice of benchmark and optimization metric. It therefore depends on the chosen configuration alone. 

{\bf \review{
D2. Definition 2.4: how exactly should we think about a workload? Is it a set of fixed queries that arrive in some order? Is it a probability distribution over queries? Or is it just a set of query templates? This is important later on, since the workload is an input to the optimization problem.}}

In our implementation, UDO only requires a script that tests a given configuration and produces a numerical performance measure to maximize. We model this script via the benchmark metric function $f$. It may internally use a fixed workload or generate queries randomly according to a fixed probability distribution. Our model assumes that $f$ is in general stochastic and therefore covers both cases. We describe several options in the revised Example~\ref{ex:benchmarks}.

{\bf \review{
D3. Definition 2.6: what does the expectation mean here? What is the probability distribution? Also, what does it mean to condition on the benchmark $B$?}}

We simplified the model and dropped the separation between benchmark $B$ and optimization metric $f$. Instead, we assume that function $f$ is now the ``benchmark metric'' (see revised Definition~\ref{def:fmetric}) and integrates the choice of benchmark as well as the performance metric to optimize. The goal of UDO is to maximize the performance values returned by $f$. 

As outlined in revised Definition~\ref{def:fmetric}, we assume that $f$ is stochastic: evaluating the same configuration twice does not yield the same performance, typically, due to different transaction calls (if $f$ relies on randomly generated workloads) or to various noise sources (e.g., caching effects, changes in system load) that influence the run time of queries and transactions. As $f$ is stochastic, our goal is to find the configuration with maximal average performance (i.e., expected value of performance metric).

% The performance of a configuration under a benchmark $B$ varies among different runs. The expectation is empirical mean of performance among multiples runs. It is condition on the benchmark $B$ because for different benchmark, the performance of a fix configuration is different. And we would like to find a fix configuration for the given benchmark $B$.

{\bf \review{
D4. Definition 2.7: This definition is not very clear. For example, what exactly is an episodic MDP? How does the reward function come into the picture? Some background on MDPs would be useful here.}}

We added a formal definition of episodic MDPs in Section~\ref{sec:model}. We also rewrote the definitions of the two UDO-specific MDPs.

% A MDP, defined by a tuple $\langle\mathcal{S},\mathcal{A},\mathcal{T},\mathcal{R}\rangle$. $\mathcal{S}$ is the state space, $\mathcal{A}$ is the finite action space and $\mathcal{T}:\mathcal{S}\times\mathcal{A}\mapsto\mathcal{S}$ is the transition
% function. Normally an episodic MDP specifies two additional parameters, horizon $H$ and max episode $N$. 
% And the agent start from episode $0$ to $N$, in each episode, the agent start from an initial state, normally defined as $s_0$, takes an action, gains a reward and moves to next state. The agent can take at most $H$ steps.

{\bf \review{
D5. Definition 2.8: I don't understand how $C_H$ and $C_L$ are defined. Are they subsets of $C$? If so, how can one specific configuration be classified as light or heavy since what matters is the change - and not the state by itself?}}

Strictly speaking, $C_H$ and $C_L$ are not subsets of $C$. Instead, $C_H$ represents all possible settings for heavy parameters and $C_L$ all possible settings for light parameters. Hence, as light and heavy parameters are disjunct, space $C$ corresponds rather to the cross product between $C_L$ and $C_H$: $C=C_H\times C_L$. We added more details in Definition~\ref{def:heavylight}. 

{\bf \review{
D6. Definitions 2.7 - 2.11: this part can be presented in a much more concise way.}}

We removed one definition (of simple MDPs) and rewrote the other definitions, shortening them while reducing formalisms to a minimum.

%\textcolor{red}{Todo. DB: Edited the definitions a bit specially 2.8. Please have a look.} 

{\bf \review{
D7. Example 2.12: a figure here would help a lot.
}}

We replaced that example with Example~\ref{ex:mdps} in the revised version which is associated with Figure~\ref{fig:mdp} (a slightly adapted version of an example that previously appeared much later in the paper).

{\bf \review{
D8. Section 4: how exactly is the split between heavy and light decided? If this is not specified by the user, how does the algorithm decide what parameters are hard to change?
}}

We currently distinguish parameters simply based on the parameter type. We outline the details in the text below Definition~\ref{def:heavylight}.


{\bf \review{
D9. Theorem 7.1: what is the Reconfiguration problem? If you claim it is NP-hard, it should be presented formally. Otherwise, the theorem statement is imprecise.
}}

% The Reconfiguration problem is defined, given a configuration list $C_h = \{ c_1, c_2, \cdots, c_l \}$ with length $l$ and a $\text{cost}$ function mapping from a specific configuration to its creation cost, our goal is to find a permutation of configuration list $C$, denoted as $\bar{C} = \{ \bar{c}_1, \bar{c}_2, \cdots, \bar{c}_l \}$, such that the total cost of $\bar{C}$, $\sum_{t=1}^{l} \bar{c}_t - \sum_{t=1}^{l-1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$ is minimized. This problem is same as maximizing the overlapping cost, $\sum_{t=1}^{l - 1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$. 

We added a formal definition of that problem (Definition~\ref{def:orderingproblem}).

%The Reconfiguration problem is defined, given a configuration list $C_h = \{ c_1, c_2, \cdots, c_l \}$ with length $l$ and a cost metric $c_{i,j}$ indicating the cost of switching from configuration $i$ to configuration $j$, the goal is to find a permutation function $\Pi$ that maps positions from 1 to $l$ to indices from 1 to $l$, to minimize the total Reconfiguration cost, $\sum_{1\leq i<l}c_{\Pi(i),\Pi(i+1)}$. Please refer to section ~\ref{sec:ordering} for more details. 

{\bf \review{
D10. Section 10.1: the exact parameter space should exist somewhere in order to facilitate reproducibility.
}}

We list all parameters in the appendix of our extended technical report. %attach the parameter space in the Appendix ~\ref{sec:parameter_space}.

% We added the list of parameters to the appendix of our extended technical report, available at \url{https://github.com/OVSS/UDO}.

% \textcolor{red}{Todo, important, where should include those parameters}

{\bf \review{
D11. Section 10.1: how is the workload sampling done to estimate the reward?
}}

We added more details on how we sample configuration quality in the experimental setup section (now Section~\ref{sub:expsetup}).

%\textcolor{red}{New, the system first analyzes what are applicable queries for given index configurations (i.e., system only considers queries which can be used for given indexes), it samples queries from applicable queries according to a predefined sample rate.}
% Given an index configuration to evaluate, we only consider queries  

{\bf \review{
D12. Section 10: it would be interesting to compare UDO against specialized tuning systems. For example, how does UDO compare to one of the index tuners if this is the only thing we want to optimize?
}}

We compare UDO to multiple specialized tools for the problem of index tuning in the newly added Figure~\ref{fig:tpch_index_tune_benchmarks}. Thank you for the suggestion.

%show index selection results in Figure ~\ref{fig:tpch_index_tune_benchmarks}. In this experiment, we fix the system parameter as the default system parameter for both Postgres and MySQL. For UDO, DDPG and SARSA, the goal is to recommend three indexes (top-3 index selection). It is clear that UDO are better than all baselines.

% We add top-k index selection experiments on TPC-H of scaling factor one and scaling factor ten. 

{\bf \review{
D13. Section 10: what would happen if we used cost estimators instead of running the workload? I assume that the running time would be faster, but how much would we lose in terms of performance? This is an important baseline.
}}

We added a baseline that uses the optimizer cost model for index recommendations in the experiments shown in Figure~\ref{fig:tpch_index_tune_benchmarks}. The quality of the proposed solution is lower.

%Changes of many light configurations (e.g., transaction order, buffer pool size and parallel workers) may not captured by statistics of optimizer. We add a baseline for index recommendation using the cost optimizer, named Brute-force Cost Model in Figure ~\ref{fig:tpch_index_tune_benchmarks}. The Brute-force Cost Model approach enumerates all three indexes combinations and returns the one having smallest estimated cost.

{\bf \review{
D14. Section 10: how would UDO work if there was not a given time limit? For example, suppose that we wanted to optimize until no further improvement is seen. Can the algorithm be modified to work in this way? This is important since it is not clear how the user can come up with an appropriate time limit. E.g., if the scale of the data increases, how much more time should we give to UDO?
}}

The algorithm can definitely be modified in that way. For example, we can detect the improvement between episodes and terminate, once the improvement for a configurable number of episodes is below a configurable threshold. We can also measure how long it takes until we don't have any improvements of more than x\% for y consecutive episodes where $x$ and $y$ are inputs of the algorithm. We added a corresponding remark in Section~\ref{sec:overview} (see footnote).

We also added experiments in which we increase the data size for TPC-H (e.g., see Figure~\ref{fig:tpch_sf10_benchmarks}).

%For the performance of UDO as the increase of the data increases, we add the TPC-H experiments with scaling factor ten, show in Figure ~\ref{fig:tpch_sf10_benchmarks}.

==> revision/reviewer2.tex <==
\begin{center}
\line(1,0){240}
\end{center}

\subsection*{\huge Review 2 Details} 

{\bf \review{
D1. While the general intuition is clear, the structure and figures not really make it easy to understand the core components and how they interact.
}}
 
We improved the presentation as outlined below.
 
{\bf \review{D2. In the first pages the main intuition of heavy and light parameters is repeated multiple times which is not required.}}

We removed the repeated introduction of heavy and light parameters in Section~\ref{sec:overview}.

{\bf \review{D3. This is important: The system overview (the text in Section 3 as well as Figure 1) is not really helpful in understanding the interplay of components (e.g., what is happening when?). Please add a new figure and rewrite this section since then the rest of the paper might be easier to read.}}

We added a new figure and rewrote Section~\ref{sec:overview} from scratch.


{\bf \review{
D4. Also Sections 4-9 need a better structuring. Some seem to be subsection e.g. picking and planning. Moreover, cross-references in algorithms are very implicit. Please make clear which function will be detailed in a following section.
}}

We restructured those sections by merging former Section~4 with Section~3, making the former ``picking'' and ``planning'' sections subsections of a new section, and by making cross-references between algorithms more explicit (e.g., we point out at the beginning of Sections~\ref{sub:picking} and \ref{sub:ordering} where the presented algorithms are invoked).

{\bf \review{
D5. Why would an approach with a normal RL agent that simply keeps a physical configuration for heavy parameters (and does not simply drop it) once it was created and simply reuses the database files later once the same heavy configuration is selected ...}}

%by the RL agent again. Keeping a physical configuration is trivial in DBMS (also in Postgres and MySQL) since often a DB is simply a bunch of files that can be linked into the database. Hence, reconfiguration is for free if the configuration was created once. The paper should compare to such a much simpler strategy which uses normal RL with caching of the physical configurations. This should be slower at the beginning but eventually then improve faster than UDO once many configurations are cached.

Caching is only useful if the exact same configuration is selected repeatedly (e.g., if we want to evaluate performance of a specific index set, we cannot reuse a configuration featuring a superset of those indexes as the sheer presence of indexes that need to be updated influences performance). UDO's evaluation order optimization mechanisms reduce cost already when selecting configurations with similar index sets within the delay time window. There are some overheads in copying physical configurations and storage space becomes a bottleneck as the number of cached configurations grows. In any case, we agree that this would be an interesting comparison and have added a corresponding baseline (``RL with Cache''), for instance in Figures~\ref{fig:tpch_benchmarks} and \ref{fig:tpch_sf10_benchmarks}. Thank you for the suggestion.

%For the TPC-H, the number of indexes candidate is 99. If we cache all the combination of indices, the possible number of choice is $9.332622 \times {10}^{155}$. For the TPC-H scaling factor 1, the space consumption is $1.399893 \times {10}^{156}$ GB, which is impossible to save in the disk. We add a new baseline named Cache in Figure \ref{fig:tpch_benchmarks}, \ref{fig:tpch_sf10_benchmarks} and \ref{fig:tpcc_benchmarks}. For TPC-H, we create 100 (around 150G) TPC-H database copies with scaling factor 1 and 20 (more than 220G) TPC-H database copies with scaling factor 10. And if a sampled heavy configuration generated from RL agent is cached by one database, it chooses the corresponding database to evaluate light configurations. If a sampled heavy configuration is not cached and there are available free databases, it chooses one free database and build the sampled heavy configuration. If a sampled heavy configuration is not cached and there are no free databases, it randomly chooses a database and overrides the heavy configuration of the selected database.

% We run the following experiments on TPC-H with scaling factor one and scaling factor ten. We create 100 (around 150G) TPC-H database copies with scaling factor 1 and 12 (around 150G) TPC-H database copies with scaling factor 10.

% We run the following experiments on TPC-H with scaling factor one and scaling factor ten. We create 100 (around 150G) TPC-H database copies with scaling factor 1 and 12 (around 150G) TPC-H database copies with scaling factor 10. And if the generated indices is cached, we use the cached indices otherwise we randomly pick up a copy, drop the previous indices and build new selected indices. 


{\bf \review{
D6. The parameter for changing statement orders in transactions seems a very limited form of transaction scheduling. Are there not more interesting tuning knows such as number of worker threads which might have a strong influence especially when it comes to low- and high-conflicting workloads.
}}

We include several tuning knobs that refer to the degree of parallelism (e.g., \verb|max_parallel_workers| and \verb|max_parallel_workers_per_gather|). We optimize those and the order of operations within transaction templates. Prior work has shown that the latter type of optimization has significant impact on performance as well~\cite{Yan2016}. We include the list of optimized parameters in the appendix of our extended technical report~\cite{Wang2021c}.% \revision{TODO: add reference to online report}

%The number of client request threads more depends on the hardware of client. We fix it in the TPC-C experiments. 
%We include the concurrency (work threads) related system parameters as light parameters, such as \textit{max\_parallel\_workers}, \textit{max\_parallel\_workers\_per\_gather} and \textit{innodb\_thread\_concurrency}.

{\bf \review{
D7. Moreover, important questions such as database updates need to be discussed more carefully especially if OLTP is a target since the database might significantly grow over time which might change what is the optimal configuration. How is this being incorporated into the learning? At least a discussion is needed why this does not seem to matter.
}}

This is generally a challenge with OLTP database tuning, e.g.\ see Question~4 in OtterTune's Wiki~\footnote{https://github.com/cmu-db/ottertune/wiki/FAQ}. We adopt the same solution as OtterTune, according to that Wiki: we periodically reload the database. We added a corresponding remark in Section~\ref{sub:expsetup}.

%Like many prior works \cite{Zhang2019a}, to avoid the change of optimal configuration as a database grows, we reset the database to its initial status after a fix tuning period. 

{\bf \review{
D8. Section 7: It is not clear to me how the graph is constructed and what edges mean in this graph.
}}

Nodes represent configurations to evaluate. Edges represent the cost for switching from one configuration to another one (e.g., by creating and dropping indexes). We added a formal problem definition in Section~\ref{sub:ordering} to clarify semantics.

% The graph with nodes and edges are not construed, instead they are the input of hamiltonian path problem. To prove the Reconfiguration problem is a NP-hard problem, we assume there exists a Reconfiguration solver, it can be used to solve the hamiltonian path problem. The construction procedure is shown in ~\ref{pf:reconfiguration}. 

{\bf \review{
D9. This is important: The paper seems to rely on the knowledge the reconfiguration cost to switch from one to another configuration upfront. This seems unrealistic. How could the approach work without this information? Did I misunderstand something here?
}}

We could measure time for switching each knob in a (admittedly expensive) pre-processing step. Instead, we use a simple proxy: we only consider cost for index creations and approximate it by the cardinality of the table being indexed. While not precise, this metric is sufficient to make cost-based optimization beneficial (e.g., see Figure~\ref{fig:delay}). We added a remark on this in Section~\ref{sub:ordering}.

%Indeed, we cannot know the precise cost (e.g., for index creations) a-priori which is also subject to some random variations. However, we use estimates as a proxy. For index creations, we estimate cost as the cardinality of the indexed table. While this is of course imprecise, it is close enough to make cost-based optimization beneficial (see Figure~\ref{fig:delay}).

%We use the cardinality to estimate the creation cost of indexes. 

{\bf \review{
D10. The experiments lack important details especially when it comes to OLTP. How is the transaction mix being executed? Are clients randomly selecting the transactions given the mix of TPC-C or is the execution more deterministic?
}}

%For TPC-C, transactions are mixed with 4\% \verb|STOCK_LEVEL|, 4\% \verb|DELIVERY|, 4\% \verb|ORDER_STATUS|, 43\% \verb|PAYMENT| and 45\% \verb|NEW_ORDER|.

%Clients randomly select transactions given the mix probability of TPC-C workload. 

We added details on the TPC-C transaction mix in Section~\ref{sub:expsetup}.

{\bf \review{D11. For OLTP, many other physical parameters such as the maximum number of concurrent worker processes / threads might be interesting to tune. The selection of the tuning parameters for OLTP should be done more carefully.}}

We consider several parameters concerning number of workers/threads, e.g., for Postgres, \verb|max_parallel_workers|, \verb|max_parallel_workers_per_gather|, and, for MySQL, \verb|innodb_thread_concurrency|. The complete list of parameters tuned can be found in the appendix of our extended technical report~\cite{Wang2021c}. 


%The number of client request threads more depends on the hardware of client. We fix it in the TPC-C experiments. We include the concurrency (work threads) related system parameters as light parameters, such as \verb|max_parallel_workers|, \verb|max_parallel_workers_per_gather| and \verb|innodb_thread_concurrency|.


{\bf \review{
D12. The evaluation also would benefit from using databases with more realistic sizes (especially when it comes to TPC-H).
}}

We agree and have added experiments with scaling factor 10 for TPC-H (e.g., see Figure~\ref{fig:tpch_sf10_benchmarks}).

%We add TPC-H experiments with scaling factor ten, shown in Figure \ref{fig:tpch_sf10_benchmarks}

{\bf \review{
D13. Include other baselines (as suggested in D5) in the experiments.
}}

We have added the requested baseline, please see our answer to D5 for details.

%For the TPC-H, the number of indexes candidate is 99. If we cache all the combination of indices, the possible number of choice is $9.332622 \times {10}^{155}$. For the TPC-H scaling factor 1, the space consumption is $1.399893 \times {10}^{156}$ GB, which is impossible to save in the disk. We add a new baseline named Cache in Figure \ref{fig:tpch_benchmarks}, \ref{fig:tpch_sf10_benchmarks} and \ref{fig:tpcc_benchmarks}. For TPC-H, we create 100 (around 150G) TPC-H database copies with scaling factor 1 and 20 (more than 220G) TPC-H database copies with scaling factor 10. And if a sampled heavy configuration generated from RL agent is cached by one database, it chooses the corresponding database to evaluate light configurations. If a sampled heavy configuration is not cached and there are available free databases, it chooses one free database and build the sampled heavy configuration. If a sampled heavy configuration is not cached and there are no free databases, it randomly chooses a database and overrides the heavy configuration of the selected database.



==> revision/reviewer3.tex <==
\begin{center}
\line(1,0){240}
\end{center}

\subsection*{\huge Review 3 Details} 

{\bf \review{
D1. The paper forces the user to define a (static) quantitative reward function over a sample workload. Such a function could neglect side effects in terms of resource consumption, contention, or durability if they are not included in the metric. In other words, the concept of a universal database optimizer means that there is a universal database numerical SLO.
}}

Please note that we can optimize for composite performance metrics, integrating multiple other metrics. E.g., we added experiments in which we optimize a weighted sum between query execution time and disk space (see newly added Figure~\ref{fig:spaceplustime}). 

{\bf \review{
D2. Comparison with OtterTune. As this is the most high-profile recent work in this space, I was a little disappointed in the author's discussion of it.
-D2.1 There is no quantitative comparison between OtterTune and UDO. It is definitely possible: https://dl.acm.org/doi/10.14778/3229863.3236222
-D2.2 One of the key contributions of OtterTune is adaptivity to changing workloads. UDO does not support this. It's a mischaracterization to call UDO a "more ambitious" proposal.
}}

We removed the reference to ambition in Section~\ref{sec:related}, thank you for the suggestion. OtterTune, a highly visible and seminal work in this space, focuses on tuning database system parameters while we additionally make e.g.\ indexing choices. We added OtterTune as well as the recently proposed DDPG++ algorithm as baselines for many of our experiments (D2.1) and added a comparison on a changing workload (D2.2). 

%We agree that our characterization of UDO as ``more ambitious'' was misplaced. We have removed that term in our revision (TODO!). We just meant that UDO considers some classes of optimization parameters, namely index selections and transaction template changes, that OtterTune does not consider. 

%We added OtterTune, as well as the recently proposed DDPG++ algorithm, as baselines for our experiments (see Figures~\ref{fig:tpcc_benchmarks}, \ref{fig:tpch_benchmarks}, and \ref{fig:tpcc_benchmarks}).

%We add the OtterTune-DDPG+ and OtterTune-GP as a baseline for all experiments, show in Figure ~ \ref{fig:tpch_benchmarks}, ~\ref{fig:tpch_sf10_benchmarks} and ~\ref{fig:tpcc_benchmarks}.

{\bf \review{
D3. The need for a universal optimizer is also not well justified. What if the authors combined an index advisor with a system configuration tuner, what performance would that get?
}}

We agree that this is an interesting comparison - we have results in which we combine recommendations by different tools for separate sub-problems (e.g., see baseline QURO+Dexter+PGTuner in Figures~\ref{fig:tpcc_benchmarks} and \ref{fig:tpch_benchmarks} which combines transaction templates proposed by QURO with indexes recommended by Dexter and configuration parameters recommended by PGTuner as well as other combined baselines). Using a single tool also facilitates using composite optimization objectives (e.g., optimizing tradeoffs between run time, dependent on system parameters settings as well as available indexes, and disk space consumed for indexes, which we do in Figure~\ref{fig:spaceplustime}).

%Please refer to our results which combine system parameter tuning tools and index recommendation tools. Baselines of combing system parameter tuning tools (PGTune/MySQLTune) and index recommendation tools (Dexter/EverSQL) shown in Figure ~ \ref{fig:tpch_benchmarks}, ~\ref{fig:tpch_sf10_benchmarks} and ~\ref{fig:tpcc_benchmarks}.

{\bf \review{
D4. The quantitative results are actually not terribly impressive. On Figure 3/4 the y-axes are cut to make the gains seem import important. After 4 hrs of configuration search, the algorithms are all within 20\% of each other. I think this is insignificant over a static workload.
}}

Please note that the advantage may grow as the data size grows. For instance, for TPC-H with scaling factor 10 running on Postgres (see newly added Figure~\ref{fig:tpch_sf10_benchmarks}, right sub-figure), UDO is 25\% better than the best baselines (136 seconds for UDO versus 181 seconds for the second-best baseline) and the spread of run times is much larger when considering all algorithms.

%For the index recommendation, shown in Figure \ref{fig:tpch_index_tune_benchmarks}, UDO is more than 25\% better than baselines.

%For the TPC-H with scaling factor 10, shown in Figure \ref{fig:tpch_sf10_benchmarks}, UDO is more than 25\% better than baselines.

{\bf \review{
D5. As I understand the algorithm, the authors use RL to plan out next configurations to search. In this sense, the actually configuration identification problem is not stateful but the search process is (you are at a current database state) ...}}

%. This is an active design decision that should be tested out more:
% - What if we used a contextual bandits approach and simply tolerated the configuration switching costs between each arm pull?
% - Could a stateless approach like the one above be more readily parallelized over multiple deployments to test configurations? Does RL preclude parallel configuration search?
% - My intuition is that bad configuration parameters are really bad, and good ones are all roughly equivalent. Could one early terminate actions that run longer than the best config already seen?

Please note: when selecting the next configurations to try, our RL algorithm \textbf{does not} take into account the current database state. The RL algorithm selects configurations to try because they seem interesting, independently of the reconfiguration cost needed to evaluate them. However, after the RL algorithm has selected configurations to try, the cost-based optimizer does its best to keep reconfiguration costs low. It can do so as the RL algorithm can deal with delay between selecting and evaluating configurations. 

We completely agree with your point that integrating reconfiguration cost into the decision about which configurations to evaluate may lead to sub-optimal solutions. This is why we do not do that! We added a corresponding remark in Section~\ref{sec:overview}.

%\textcolor{red}{Too many ideas, still do not how to address this}

{\bf \review{
D6. How much does UDO "overfit" to the sample workload?
* Vary the size of the sample workload
* Evaluate UDO under workload shifts or bursty changes in the workload
}}

% We add TPC-H experiments with scaling factor ten. We introduce the following synthetic shifting workload as follows, in the odd tuning time, system only receives odd TPC-H queries while in the even tuning time, system only receives even TPC-H queries. 

% We design two experiments to test the generalizability of UDO. 
% \begin{itemize}
%     \item We randomly select several percentage of queries as training queries in TPC-H, and test the performance of all 22 TPC-H queries, shown in Figure \textcolor{green}{Running} ~\ref{fig:postgresshiftquery}.
%     \item We initialize the TPC-H queries with 100 different seeds. In the training procedure, we randomly select several percentage of seeds as training queries, and in the testing procedure, we test the performance of all TPC-H queries with 100 seeds, shown in Figure ~ \ref{fig:postgresshiftworkload}. \textcolor{green}{Running}.
% \end{itemize}

We added two corresponding experiments in Section~\ref{sub:scenarios} (see Figure~\ref{fig:postgresdynamic}).

% \textcolor{red}{To change}

% We design the following experiments to test the generalizability of UDO. We randomly select several percentage of queries as training queries in TPC-H, and test the performance of all 22 TPC-H queries, shown in Figure ~\ref{fig:postgresshiftquery}.

{\bf \review{
D7. How does UDO affect performance metrics not captured by the reward function (i.e., not latency)?
* Measure disk/memory usage, CPU utilization, available concurrency
}}

We added more performance metrics in the appendix of our extended technical report~\cite{Wang2021c}.

% We report the disk space, memory usage and CPU utilization for final configurations of UDO in the appendix.

% \textcolor{red}{Todo list those in appendix}

{\bf \review{
D8. Comparison with OtterTune and other baselines
* Use the sample workload used for performance eval in UDO as the input to OtterTune (or any other baseline), compare CPU cycles or time or some other measure of resources needed to reach a good DB configuration.
* How much exploration is needed to periodically retrain UDO under workload shifts? Periodically retrain UDO with shifting workloads, compare to OtterTune in this setting.
}}

We added a comparison against OtterTune throughout our experiments and also experimented with shifting workloads (see Section~\ref{sub:scenarios}).

% For the comparison of UDO and OtterTune + dexter in the static workload setting, please refer to Figure ~ \ref{fig:tpch_benchmarks}, ~\ref{fig:tpch_sf10_benchmarks} and ~\ref{fig:tpcc_benchmarks}.

% \textcolor{red}{To change}

% For the comparison of UDO and OtterTune + dexter in the dynamic workload setting, please refer to Figure ~\ref{fig:postgresdynamic}.

% We add experiments of shifting workloads for the TPC-H benchmark.

==> sections/analysis.tex <==
\section{Theoretical Analysis}
\label{sec:analysis}

%In this section, we prove convergence of Dealyed-HOO without RAVE updates, and UDO framework using it for solving both heavy and light parameter UDO MDPs. 

We show, under moderately simplifying assumptions, that UDO converges to optimal configurations. UDO uses an extension of HOO algorithm, which provides this type of guarantee (Theorem 6,~\citep{bubeck2011a}). However, we decompose our search space (into a space for heavy and one for light parameters) and delay evaluation feedback (to amortize re-configuration costs). In this section, we sketch out our reasoning for why those changes do not prevent convergence. We provide a more detailed version of the following proofs  online\footnote{\url{https://www.cs.cornell.edu/database/supplementary_proofs.pdf}}. 

In doing so, we use \textit{expected regret}~\citep{Auer2002} as the metric of convergence. Given a time horizon $T$, expected regret $\mathbb{E}[\reg_T]$ is the sum of differences between the expected performance of the optimal configuration and the configuration achieved by the algorithm at any time step $t \leq T$. If the expected regret of an algorithm grows sublinearly with horizon $T$, it means the algorithm asymptotically converges to optimal configuration as $T \rightarrow \infty$.
% We discuss several reinforcement leaning algorithm here and provide the regret bound for the aforementioned two level reinforcement learning algorithm. We utilize the delay HOO and delay EXP3 tree search as the underlying delay reinforcement learning model. 
\begin{theorem}[Regret of HOO (Theorem 6,~\cite{bubeck2011a})]\label{thm:HOO}
If the performance metric $f$ is smooth around the optimal configuration (Assumption 2 in~\citep{bubeck2011a}) and the upper confidence bounds on performances of all the configurations at depth $h$ create a partition shrinking at the rate $c\rho^h$ with $\rho \in (0,1)$ (Assumption 1 in~\citep{bubeck2011a}), expected regret of HOO is
\begin{align}\label{eq:hoo}
    \mathbb{E}[\reg_T] = O\left(T^{1-\frac{1}{d+2}}(\log T)^{\frac{1}{d+2}}\right)
\end{align}
for a horizon $T > 1$, and $4/c$-near-optimality dimension\footnote{$c$-near-optimality dimension is the smallest $d\geq 0$, such that for all $\varepsilon > 0$, the maximal number of disjoint balls of radius $c\varepsilon$ whose centres can be accommodated in $\mathcal{X}_\varepsilon$ is $O(\varepsilon^{-d})$ (Def. 5 in~\citep{bubeck2011a}). Here, $\varepsilon$-optimal configurations $\mathcal{X}_\varepsilon \triangleq \{ x \in C | f(x) \geq f^* - \varepsilon\}$.
Near-optimality dimension encodes the growth in number of balls needed to pack this set of $\varepsilon$-optimal configurations as $\varepsilon$ increases.} $d$ of $f$.
\end{theorem}
Typically, configuration space $C$ is a bounded subset of $\mathbb{R}^P$ and performance metric $f:C \rightarrow [a,b] \subset \mathbb{R}$. Here, $d$ is of the same order as the number of parameters $P$. HOO uses UCB1~\cite{Auer2002} rather than UCB-V~\citep{ucbv}. For brevity of analysis, we follow the same though the proof technique is similar for any UCB-type (Upper Confidence Bound) algorithm.

\subsection{Regret of Delayed-HOO}
Now, we prove that using delayed-UCB1~\citep{Joulani2013a} instead of UCB1 allows us to propose delayed-HOO and also achieves similar convergence properties.
%We prove convergence properties of the Delayed-HOO algorithm which can be used inside of the UDO framework.
\begin{theorem}[Regret of Delayed-HOO]\label{thm:delayed-HOO}
Under the same assumptions as Thm.~\ref{thm:HOO}, the expected regret of delayed-HOO is 
\begin{align}\label{eq:delayed_hoo}
    \mathbb{E}[\reg_T] = O\left((1+\tau)T^{1-\frac{1}{d+2}}(\log T)^{\frac{1}{d+2}}\right)
\end{align}
for delay $\tau \geq 0$, horizon $T$, and $4/c$-near-optimality dimension $d$ of $f$. 
\end{theorem}
\begin{proof}[Proof Sketch]
First, we observe that for delayed-HOO, we can decompose the regret into two terms: one as same as the original HOO and the other one for delay. This decomposition holds true because by Theorem in~\citep{Joulani2013a}, we can decompose the delay-dependent and independent components of regret for delayed-UCB1. 
The delay-independent term leads to the same result as Eq.~\eqref{eq:hoo}.
The delay-dependent term reduces to $\sum_{h=1}^{Depth(MCT)} \rho^{h(2-d)} \tau$. 
If we follow the proof of HOO, we obtain this term is $O(\tau T^{-\frac{d}{d+2}}(\log T)^{\frac{d}{d+2}})$ for $\rho^{Depth(MCT)} = O(T/\log T).$ 
Since $\log T/T < 1$ for all $T \geq 1$, we obtain that $\mathbb{E}[R_T(c)] \leq O(((1+\tau)T^{1- \frac{1}{d+2}}(\log T)^{1/(d+2)})$.
\end{proof}
The bound in Eq.~\eqref{eq:delayed_hoo} is the same as Eq.~\eqref{eq:hoo} with an additional factor $(1+\tau)$, which does not change the convergence in terms of $T$. For delay $\tau = 0$, we retrieve the regret bound of original HOO.

The expected error in estimated expected performance (or reward) of any given configuration at time $T$ is $r(T) = \mathbb{E}[f^* - \hat{f}(c_T)] = \frac{1}{T}\mathbb{E}[\reg_T]$.
Thus, the expected error $\epsilon(T)$ in estimating the expected performance (or reward) of a configuration using delayed-HOO converges at the rate $O\left((1+\tau) \left[\log T/T\right]^{1/(d+2)}\right)$, where $T$ is the number of times the configuration is evaluated. 






% It is well-known that the HOO algorithm balances between exploration and exploitation in a principled manner that results in probabilistic guarantees. However, the traditional HOO algorithm has to update the reward of the selected actions at each round. \cite{} proposes a UCB manner selection strategy for online algorithm under the delayed feedback. We applied this selection strategy in the Monte Carlo Search Tree, and proposed the delay HOO algorithm. In the delay HOO tree, the reward of each tree node is not updated immediately. Instead, the reward information of each tree node can be updated after $d$ episodes from its selection, where $d$ is the maximal delay time as the input parameter.
\iffalse
\begin{lemma}[Regret of delayed-UCB-V]\label{thm:delayed-ucbv}
For any $T \geq 1$, the expected regret of delayed-UCB-V with delay $\tau$ (Eq.~\eqref{eq:delayeducbv}) is bounded by
\begin{align*}
    \mathbb{E}[\reg_T] \leq 10 \sum_{i: \Delta_i > 0} \left[ \left( \frac{\sigma_i^2}{\Delta_i} + 2b \right) \log T + \tau \Delta_i. \right]  
\end{align*}
Here, $\sigma_i^2$ is the variance of rewards for action $i$, $\Delta_i$ is the difference in expected rewards of the optimal action and action $i$, and $b>0$.
\end{lemma}
\begin{proof}[Proof Sketch]
Following the proof of Theorem 7~\citep{Joulani2013a}, we decompose the expected regret of delayed-UCB-V in two terms. The first term is the regret term appearing due to use of UCB-V itself. The second term is due to the error in computed statistics due to delayed feedback. We can bound them individually using the UCB-V regret bound~\citep{ucbv} and delay times the suboptimality of rewards of all the actions, i.e.\ $\tau \sum_{i} \Delta_i$. By combining these, we obtain that the expected regret of delayed-UCB-V is $O(\log T + \tau)$.
\end{proof}

% \deba{For the next proof, we have to change a few stuffs in delayed-HOO. First is making the B value infinity for unvisited states. Second is modifying the selection process to $b_{p}(t) = \min\{\text{UCB-V equation for conf at }(p) + \rho^{depth(p)}, \max_{c \in C(p)} b_p(t)\}$. This framework of MCTS is called Hierarchical Optimistic Optimization (HOO)~\citep{bubeck2011a}.}

\begin{theorem}[Estimation Bias of Delayed-HOO]\label{thm:delayed-HOO}
Under the same assumptions as HOO, the error in the expected value of any state $s$ as estimated by delayed-HOO is bounded by $O\left((1+\tau) \left[\log T/T\right]^{1/(d+2)}\right)$ for a delay $\tau > 0$, horizon $T$, and $4/c$-near-optimality dimension $d$ of $f$. 
\end{theorem}
\begin{proof}[Proof Sketch]
The error in estimated expected reward of a given configuration at time $T$ is $r_T(c) = \frac{1}{T}\mathbb{E}[R_T(c)]$. By generalising Theorem 6 in~\citep{bubeck2011a}, we obtain that if delayed-UCB-V algorithm with expected regret bound $O(\log T + \tau)$ is used in HOO framework, $\mathbb{E}[R_T(c)] \leq O(((1+\tau)T^{\frac{d+1}{d+2}}(\log T)^{1/(d+2)})$. Now using relation between error and regret, we obtain that $r_T(c) = O\left((1+\tau) \left[\log T/T\right]^{1/(d+2)}\right)$ for delayed-HOO.
\end{proof}
This shows that the error in estimating the expected performance (or reward) of a configuration using delayed-HOO (without RAVE updates) converges at the rate $O\left((1+\tau) \left[\log T/T\right]^{1/(d+2)}\right)$, where $T$ is the number of times the configuration is evaluated. 
% \subsection{Delay EXP3}
% Delay EXP3 selection strategy is proposed in \cite{} for the delay multi-arm bandit problem. Compared with UCB, it adopts the probabilistic policies instead of deterministic policies, 
% % The advantage of EXP3 compared with UCB selection strategy is that 

% \begin{theorem}
% For the delay EXP3 algorithm, the expected regret is bounded by $O()$
% \end{theorem}
\fi

\subsection{Regret of UDO}
As we have obtained the error bound of the delayed-HOO algorithm, now we can derive bounds for UDO when using delayed-HOO for heavy and light parameters with two different delays.

\begin{theorem}[Regret of UDO]\label{thm:udo}
If we use the delayed-HOO as the delayed-MCTS algorithm with delays $\tau$ and $0$, and time-horizons $T_h$ and $T_l$ for heavy and light parameters respectively, the expected regret of UDO is upper bounded by \begin{align}\label{eq:udo}
    \mathbb{E}[\reg_T] = O\left((1+\tau)T_h^{1-\frac{1}{d+2}}(\mathrm{HOO}^2(T_l) \log T_h)^{\frac{1}{d+2}}\right),
\end{align} 
under the assumptions of Thm.~\ref{thm:HOO}. Here, $\mathrm{HOO}(T_l) \triangleq O\left(\left[\log T_l/T_l\right]^{\frac{1}{d+2}}\right)$.
\end{theorem}
\begin{proof}[Proof Sketch]
The proof for UDO is similar to bounding regret for delayed-HOO on the heavy parameters' configuration space, where the rewards are observed with some estimation error. 
The estimation error $\mathrm{HOO}(T_l)$ is unavoidable due to the error in solving light parameter MDP using HOO with no delay. By Theorem~\ref{thm:HOO}, $\mathrm{HOO}(T_l) = O([\log T_l/T_l]^{1/(d+2)})$.

Now, we prove the regret bound in two steps. 
First, like in the delayed-HOO proof, we decompose the regret of UDO in three error terms due to original HOO, delay-dependent error, and estimation error for light parameters. 
Then, we plug-in the regret bounds of HOO, delay times suboptimality of expected reward of actions, and bias $\mathrm{HOO}(T_l)$ induced by HOO as obtained for light parameter MDPs. 
Now, performing algebraic manipulation leads to the regret bound where the delay factor $(1+\tau)$ and squared error $\mathrm{HOO}^2(T_l)$ appear as multiplicative factors. 
\end{proof}
\textit{Deviation in expected performance of the configuration returned by UDO from the optimum is} $O\left((1+\tau)\left[\mathrm{HOO}^2(T_l) \mathrm{HOO}(T_h)\right]^{\frac{1}{d+2}}\right)$. Here, $T_h$ and $T_l$ are the number of steps allotted for the heavy and light parameters respectively. 
Deviation in expected performance of the configuration selected by UDO vanishes as $T_h, T_l \rightarrow \infty$.
%
% We prove the convergence rate of our algorithm
% \begin{theorem}
% Convergence speed: If we plugin the delay HOO as the delay reinforcement learning model, and HOO as the non-delay reinforcement learning model, the algorithm coverage to the best configuration after episode.
% \end{theorem}





==> sections/evaluation.tex <==
\section{Evaluating Configurations}
\label{sec:evaluation}

\begin{algorithm}[t!]
\caption{EVAL: Functions for evaluating configurations.}
\label{alg:evalVar}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \Comment{Global variable representing evaluation requests}
\State $R\gets\emptyset$
\vspace{0.15cm}
\State \textbf{Input:} heavy configuration $c_H$ to evaluate and time $t$
\State \textbf{Effect:} adds new evaluation request 
\Procedure{EVAL.Submit}{$c_H,t$}
\State $R\gets R\cup\{\langle c_H,t\rangle\}$
\EndProcedure
\vspace{0.25cm}
\State \textbf{Input:} RL algorithm $\alg_L$, benchmark $B$, time $t$, and space $C_L$
\State \textbf{Output:} evaluated configurations with reward values
\Function{EVAL.Receive}{$\alg_L,B,C_L,t$}
\State \Comment{Choose configurations from $R$ to evaluate now}
\State $N\gets$\Call{PickConf}{$R,t$}
\State \Comment{Remove from pending requests}
\State $R\gets R\setminus N$
\State \Comment{Prepare evaluation plan}
\State $P\gets$\Call{PlanConf}{$N$}
\State \Comment{Collect evaluation results by executing plan}
\State $E\gets\emptyset$
\For{$s\in P.steps$}
\State \Comment{Prepare evaluation of next configurations}
\State \Call{ChangeConfig}{$s.hconf$}
\State \Comment{Find (near-)optimal light parameter settings}
\State $c_L\gets$\Call{RL.Optimize}{$\alg_L,s.hconf,C_L,B$}
\State \Comment{Take performance measurements on benchmark}
\State $b\gets$\Call{B.evaluate}{$s.hconf,c_L$}
\State \Comment{Add performance result to set}
\State $E\gets E\cup\{\langle c_L,s.hconf,b\rangle\}$
\EndFor
\State \Comment{Return evaluation results}
\State \Return{$E$}
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

The evaluator benchmarks configurations for a given benchmark. Instead of evaluating configurations in the order in which they are selected, it aims to minimize re-configuration overheads via smart scheduling. The following example illustrates the principle.


\begin{example}
We describe configurations by vectors in which each vector component represents a parameter value. Assume we have to evaluate configurations $(1,1,16MB)$, $(0,0,12MB)$, and $(0,1,16MB)$. Here, the first two components indicate whether two specific indexes are created or not, the third component represents the (configurable) amount of working memory. Assume that the latter parameter requires a server restart with a duration of 10 seconds to take effect. For simplicity, we assume that creating an index takes 20 seconds while dropping one is free. Evaluating the configurations in the given order creates (pure configuration switching) overheads of $2\cdot 20+10+10+20+10=90$ seconds (assuming that no indexes are initially created and an initial setting of $8MB$ for memory). If we evaluate them in the order $(0,0,12MB)$, $(0,1,16MB)$, and $(1,1,16MB)$ instead, those overheads reduce to $10+10+20+20=60$ seconds. Relative savings tend to increase with the size of configuration batches.
\end{example}

Pseudo-code for the evaluator component is described in Algorithm~\ref{alg:evalVar}. The evaluator interface offers two functions, represented in Algorithm~\ref{alg:evalVar}. First, it accepts evaluation requests (\textproc{EVAL.Submit}), allowing to submit configurations for evaluation, together with an evaluation deadline. Second, it allows triggering evaluations via the \textproc{EVAL.Receive} function. 
Algorithm~\ref{alg:evalVar} maintains a global variable $R$ (whose state persists across different calls to the two interface functions). This variable contains pending requests for evaluating specific configurations. Each configuration to evaluate is only partially specified (i.e., it assigns values to a subset of configuration parameters). More precisely, configurations to evaluate only contain specific values for heavy parameters. It is the task of the evaluator component, to fill in values for light parameters in order to accurately assess the potential of the heavy parameter settings. Items in $R$ correspond to tuples, combining a heavy parameter configurations with an evaluation deadline. This deadline specifies the latest possible time (measured as the number of main loop iterations, as per Algorithm~\ref{alg:twoLevelVar}) at which evaluation results must be generated. The submission function (Procedure~\textproc{EVAL.Submit}) simply adds one more tuple to set variable $R$.

Calling Function~\textproc{EVAL.Receive} triggers evaluation of a subset of pending configurations. It is up to the evaluator itself to choose, within certain boundaries, the set of configurations to evaluate. The function returns the results of those evaluations. As input, Function~\textproc{EVAL.Receive} obtains a configuration parameter $\alg_L$, specifying the algorithm to use for optimizing light parameters (for fixed  heavy parameter values). Also, it receives the benchmark $B$, the space of light parameters $C_L$, and the current time $t$ as input. The latter is important to decide which configurations must be evaluated in the current invocation.

As a first step (Line~12), Function~\textproc{EVAL.Receive} determines the set of configurations to evaluate in the current invocation. If the time $t$ has reached the deadline of any pending configurations, those configurations must be included in that set. For other configurations, the evaluator can choose to evaluate them now or to postpone evaluation. We present different variants for the corresponding decision mechanism in the following sections. Having selected configurations to evaluate, the algorithm removes those configurations from the pending set $R$. 

Having selected a set of configurations, Algorithm~\ref{alg:evalVar} decides how to evaluate them. Function~\textproc{PlanConf} selects a plan to evaluate the given set of configurations. Evaluating configurations in the right order can save significant overheads, compared to a random permutation. In particular, ordering them allows to amortize re-configuration overheads (e.g., overheads for creating an index) over the evaluation of multiple, similar configurations. The planner function (\textproc{PlanConf}) exploits this fact and aims at minimizing cost. We present multiple planning mechanisms, realizing different tradeoffs between planning overheads and result quality, in the following sections. 

After selecting a plan, Algorithm~\ref{alg:evalVar} processes the plan steps in order (loop from Line~19 to Line~28). For each plan step $s$, the system first executes re-configuration actions required to evaluate specific heavy parameter settings (Line~21). Then, it selects a (near-)optimal setting of light parameters, specifically for the current configuration of heavy parameters (Line~23). Here, we invoke a reinforcement learning algorithm described via tuning parameters $\alg_L$. We discuss alternative learning algorithms to implement this step in the following sections. Finally, Algorithm~\ref{alg:evalVar} benchmarks the current heavy and light parameter setting (Line~25) and adds the result to the set (Line~27). All evaluation results are ultimately returned to the invoking function (Line~30).

==> sections/mainalg.tex <==

\section{Main Algorithm}
\label{sec:mainAlg}

\begin{algorithm}[t!]
\caption{UDO main function.}
\label{alg:twoLevelVar}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} Benchmark \revision{metric $f$}, configuration space $C$, RL algorithms $\alg_H$ and $\alg_L$ for heavy and light parameter optimization
\State \textbf{Output:} a suggested configuration for best performance
\Function{UDO}{\revision{$f$}$, C, \alg_H, \alg_L$}
\State \Comment{Divide into heavy ($C_H$) and light ($C_L$) parameters}
\State $\langle C_H, C_L \rangle \gets$ \Call{SSA.SplitParameters}{$C$}
\State \Comment{Until optimization time runs out}
\For{$t\gets1,\ldots,\alg_H.Time$}
\State \Comment{Select next heavy parameter configuration}
\State $c_{H,t}\gets $\Call{RL.Select}{$\alg_H,C_H, c_{H, t-1}$}
\State \Comment{Submit configuration for evaluation}
\State \Call{EVAL.Submit}{$c_{H,t},t+\alg_H.maxDelay$}
\State \Comment{Receive newly evaluated light configurations}
\State $E\gets$\Call{EVAL.Receive}{$\alg_L,$\revision{$f$}$,C_L,t$}
\State \Comment{Update statistics for heavy parameters}
\State \Call{RL.Update}{$\alg_H,E$}
\EndFor
\State \Return best obtained configuration
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

%(i.e., a specific benchmark and performance metric) 

Algorithm~\ref{alg:twoLevelVar} describes the main function, executed by UDO. The input is a benchmark \revision{metric to optimize, a configuration space, and} tuning parameters, specifying RL algorithms to use for selecting heavy and light parameter settings. Those tuning parameters include properties that restrict the run time for optimization. \revision{Users only need to specify optimization time (hence, it is the only one represented in Figure~\ref{fig:process}) while defaults are available for the others.} The output of Algorithm~\ref{alg:twoLevelVar} is the best configuration observed until the optimization time limit\footnote{\revision{Instead of a fixed optimization time budget, we could use other termination criteria as well. For instance, the algorithm could terminate once a given number of iterations does not yield improvements above a configurable threshold.}}.

First, Algorithm~\ref{alg:twoLevelVar} analyzes the space of tuning parameters. Tuning parameters may represent indexing decisions as well as database system configuration parameters. By assessing the overheads required to change the setting for a specific parameter, UDO separates heavy from light parameters. Those two types of parameters will be optimized by different algorithms in the following.

Second, Algorithm~\ref{alg:twoLevelVar} evaluates promising configurations until the timeout is reached (loop from Line~7 to Line~16). Each iteration entails the following steps. First, UDO selects a promising configuration for heavy parameters (Line~9). The selection uses RL, applied to an MDP where states represent configurations and actions configuration changes. UDO uses RL algorithms that accept delayed feedback, i.e.\ algorithms that accept a delay between selecting options and receiving rewards evaluating them. The UDO pipeline can incorporate different algorithms as baselines. Hence, we represent the choice of algorithm as a tuning parameter. Next, UDO submits the heavy parameter configuration for evaluation (Line~11). 

The evaluator component (whose algorithm is discussed later) internally stores evaluation requests. Each request is characterized by a heavy configuration to evaluate, as well as by a deadline until which the evaluation result must be obtained. This deadline derives from constraints of delayed RL algorithms, limiting the gap between selecting action sequences and receiving associated rewards. Within the boundaries defined by deadlines, the evaluator has the autonomy to choose when and how to evaluate requested configurations. 

Algorithm~\ref{alg:twoLevelVar} receives evaluation results by calling the \textproc{Eval.Receive} function. This call causes the evaluator to choose configurations that can be evaluated cheaply, given the current state of the database system. The resulting set $E$ of evaluation results includes configurations, together with associated performance results. The latter measure the performance of the configuration on the input benchmark. The set of configurations received may or may not include cover the configuration submitted in the current iteration. To evaluate a setting of heavy parameters, the evaluator has to choose suitable settings for light parameters. The result returned from the evaluator, describes not only heavy configurations and performance results, but also the light parameter settings that enabled them.

Finally, evaluation results are used to update the statistics of the RL algorithm $\alg_H$, used for heavy parameters. The precise statistics to update depend on the algorithm used. In general, updating statistics will bias search towards configurations that are similar to the ones that perform well on benchmark $B$. 

\tikzstyle{hstate}=[rectangle, fill=blue!10]
\tikzstyle{lstate}=[rectangle, fill=green!10]
\tikzstyle{transition}=[->, black, thick]
\tikzstyle{mapping}=[->, black, thick, dashed]

\begin{figure}
    \centering
    \begin{tikzpicture}
        % Heavy configuration states
        \node[hstate] (root) at (0,0) {$\langle0,0,?\rangle$};
        \node[hstate] (hstate1) at (-3,0) {$\langle1,0,?\rangle$};
        \node[hstate, fill=red!50] (hstate2) at (3,0) {$\langle0,1,?\rangle$};
        % Light configuration states
        \node[lstate] (l1) at (-3,-1) {$\langle1,0,2MB\rangle$};
        \node[lstate] (l2) at (-3,-2) {$\langle1,0,10MB\rangle$};
        \node[lstate, fill=red!50] (l3) at (-1,-1) {$\langle1,0,25MB\rangle$};
        \node[lstate] (l4) at (-1,-2) {$\langle1,0,50MB\rangle$};
        \node[lstate] (l5) at (3,-1) {$\langle0,1,2MB\rangle$};
        \node[lstate] (l6) at (3,-2) {$\langle0,1,10MB\rangle$};
        \node[lstate] (l7) at (1,-1) {$\langle0,1,25MB\rangle$};
        \node[lstate, fill=red!50] (l8) at (1,-2) {$\langle0,1,50MB\rangle$};
        % Heavy transitions
        \draw[transition] (root) -- (hstate1);
        \draw[transition] (root) -- (hstate2);
        % Light transitions
        \draw[transition] (l1) -- (l2);
        \draw[transition] (l1) -- (l3);
        \draw[transition] (l1) -- (l4);
        \draw[transition] (l5) -- (l6);
        \draw[transition] (l5) -- (l7);
        \draw[transition] (l5) -- (l8);
        % Mappings
        \draw[mapping] (hstate1) -- (l1);
        \draw[mapping] (hstate2) -- (l5);
    \end{tikzpicture}
    \caption{Extract of heavy (top) and light (bottom) parameter MDPs for a space with two heavy and one light parameter. Optimal states for each MDP are marked up in red.}
    \label{fig:mdp}
\end{figure}

\begin{example}
Figure~\ref{fig:mdp} illustrates the two-level MDP, explored by Algorithm~\ref{alg:twoLevelVar}. In the illustrated scenario, the configuration space contains two heavy parameters (e.g., index creation decisions) as well as one light parameter (e.g., the maximal amount of main memory used per operator). Rectangles represent states in the figure and are annotated with configuration vectors (reporting parameter in the aforementioned order). The upper part of the figure illustrates the heavy parameter MDP (note that the light parameter is not specified). Solid lines mark transitions due to actions changing the configuration. Dashed lines mark mappings between heavy parameter states and the start state of the associated light parameter MDP. In total, the figure illustrates three MDPs (the one for heavy parameters and light parameter MDPs for two heavy configurations). Optimal states are marked up in red, showing that the optimal settings for light parameters may depend on the heavy parameter settings. Identifying optimal settings for heavy parameters requires obtaining optimal, associated settings for light parameters first.
\end{example}

==> sections/model.tex <==
\section{Formal Model}
\label{sec:model}

We introduce our problem model and associated terminology here.

\begin{definition}
A \textbf{Tuning Parameter} represents an atomic decision,  influencing performance of a database management system for a specific workload. It is associated with a (discrete) \textbf{Value Domain}, representing admissible parameter values. It may be subject to \textbf{Constraints}, restricting its values based on the values of other tuning parameters.
\end{definition}

We use the term ``parameter'' in a broad sense, encompassing system configuration parameter settings as well physical design decisions. In the following, we give examples for tuning parameters.

\begin{example}
Considering a set of candidate indices for a given database, we associate one tuning parameter with each candidate. Such index-related parameters have a binary value domain, representing whether the index is created or not. Equally, we can introduce a tuning parameter to represent the  \verb|random_page_cost| configuration parameter of the Postgres system (together with a set of values to consider). Finally, we may associate a query in a transaction template with a tuning parameter, representing the position within the template at which it is evaluated (the set of admissible positions is restricted via control flow and data dependencies).
\end{example}

\begin{definition}
Given fixed, ordered parameters, a \textbf{Configuration} $c$ is a vector, assigning a specific value to each parameter. The \textbf{Configuration Space} $C$ is the set of all possible configurations.
\end{definition}

Our goal is to find configurations that optimize a benchmark.

\begin{definition}\label{def:fmetric}
A \revision{\textbf{Benchmark Metric}} $f$ maps a configuration $c \in C$ to a real-valued performance result (i.e., $f:C\mapsto\mathbb{R}$)\revision{, which represents the performance of a configuration according to a specific metric for a specific benchmark}.
% A \textbf{Benchmark} is characterized by a \textbf{Workload} $W$ to optimize, as well as by a \textbf{Performance Metric} $f$, mapping configurations from space $C$ to real-valued performance results (i.e., $f:C\mapsto\mathbb{R}$). 
Higher performance results are preferable. \revision{We assume that $f$ is stochastic (i.e., evaluating the same configuration twice may not yield exactly the same performance).}
\end{definition}

\revision{Our definition of $f$ is deliberately generic, covering different types of benchmarks and metrics. A few examples follow.}

%Note that $f$ may be a stochastic function, realized by running a script measuring performance on a workload sample. We consider a variety of benchmarks and performance metrics.

\begin{example}\label{ex:benchmarks}
In our experiments, we \revision{use the following two benchmark metrics among others. We consider a benchmark metric $f_1$ that maps configurations to the average throughput, measured over a fixed time period, when processing TPC-C transactions generated randomly according to a fixed distribution. Also, we consider a benchmark metric $f_2$ that maps configurations to a weighted sum between disk space $d$ consumed (e.g., for created indexes) and run time $t$ of all TPC-H queries (i.e., $f(c)=-d-\sigma\cdot t$ where $c$ is a configuration and $\sigma\in\mathbb{R}^+$ a user-defined scaling factor). Both benchmark metrics are implemented as a script (a black box from UDO's perspective) that returns a numerical performance result.}
\end{example}

%\begin{example}In our experiments, we consider the TPC-C and TPC-H benchmarks. In TPC-C, the workload is specified by transaction templates and performance is measured in terms of throughput for a workload sample. In TPC-H, performance is measured by the negative of latency for a query sample. Optionally, we can normalize performance, e.g.\ by subtracting performance achieved by the default configuration.\end{example}

We present a system, UDO, that solves the following problem.

\begin{definition}
An instance of \textbf{Universal Database Optimization} is characterized by a benchmark \revision{metric $f$} and a configuration space $C$. The goal is to find an optimal configuration $c^*$, \revision{maximizing the stochastic benchmark metric $f$ in expectation (i.e., $c^*=\argmax_{c\in C}\mathbb{E}[f(c)]$).} We denote the optimal expected performance (that of $c^*$) as $f^*$.
\end{definition}

%according to the benchmark, i.e.\ $c^* \triangleq \argmax_{c \in C} \mathbb{E}[f(c)|B]$. 

% \begin{equation}
%     c^* \triangleq \argmax_{c \in C} \mathbb{E}[f(c)|B]\label{eq:udo}
% \end{equation}

%We aim for the expected value in Eq.~\eqref{eq:udo} as performance metric can be stochastic or include randomness during measurement. 

For iterative approaches, the problem specification may also include a user-defined timeout for optimization. The qualification ``Universal'' attest to the fact that our approach is broadly applicable, in terms of parameter types, workloads, and performance metrics. We formulate an UDO instance to one or multiple Markov Decision Processes (MDPs), and solve UDO using RL. In the simplest case, we transform UDO into one single MDP.

\begin{definition}\label{def:level1mdp}
Given an instance of the UDO problem, the associated \textbf{1-Level UDO MDP} is an episodic MDP, defined by a tuple $\langle\mathcal{S},\mathcal{A},\mathcal{T},\mathcal{R},\mathcal{S}_D,\mathcal{S}_E\rangle$. Here, $\mathcal{S}$ is the state space: each state represents a configuration. Thus, $\mathcal{S}\subseteq C$. $\mathcal{A}$ are actions: each action represents a change to one specific tuning parameter. \revision{In an episode, the algorithm starts from an initial state, takes an action, gains a reward, and moves to next state. State $\mathcal{S}_D\in\mathcal{S}$ is the start state for each episode, associated with the default configuration. $\mathcal{T}:\mathcal{S}\times\mathcal{A}\mapsto\mathcal{S}$ is called transition function that maps the source configurations and admissible configuration changes to the resulting configuration state.  States $\mathcal{S}_E\subseteq\mathcal{S}$ are end states, the current episode ends after reaching one of them. We define end states by a bound on the maximal number of changes to the default configurations (i.e., the maximal number of actions in an episode).} Also, an end state is reached if no configuration changes are possible. \revision{After end of an episode, the MDP begins again from a start state.} The reward function $\mathcal{R}$ is derived from \revision{the benchmark metric $f$. Reward for a given configuration quantifies its performance result according to $f$.} \revision{The MDP is solved by maximizing the total expected reward obtained over a given number of episodes (dictated by the user-defined timeout). This allows us to solve the UDO problem iteratively, while leveraging the efficient algorithms from RL.}
\end{definition}

Our approach factorizes the parameters into two classes.

\begin{definition}\label{def:heavylight}
We distinguish \textbf{Heavy} and \textbf{Light Parameters}, based on the overheads associated with changing their values. Heavy parameters have high reconfiguration overheads, light parameters have negligible overheads. \revision{We denote by $C_H$ the configuration space for heavy parameters (i.e., a set of vectors representing all possible heavy parameter settings). We denote by $C_L$ the configuration space for light parameters. Hence, the entire configuration space $C$ can be written as $C=\{c_H\circ c_L|c_H\in C_H, c_L\in C_L\} = C_H \times C_L$ (assuming that heavy parameters are ordered before light parameters and writing vector concatenation as $\circ$).}
\end{definition}

% We denote the configuration spaces for heavy and light parameters by $C_H$ and $C_L$ respectively.

\revision{Currently, UDO considers all parameters representing physical data structures such as indexes as heavy (as changing such parameters means creating or dropping the associated data structure). Also, UDO considers parameters as heavy that require a database server restart to make value changes effective. The other parameters are considered light. A configuration is concatenation of both heavy and light parameters.}

\revision{Depending on this categorization of heavy and light parameters, now we derive a hierarchical 2-level formulation of UDO MDP. The first level includes solving a heavy parameter MDP (Definition~\ref{def:heavymdp}), where each heavy parameter configuration is evaluated with its best light parameter configuration counterpart. The second level aims to solve a light parameter MDP (Definition~\ref{def:lightmdp}) for a given configuration of heavy parameters.}
%The definition of what constitutes ``high overheads'' is a tuning decision. In our current implementation, we simply assume that parameters related to index creations and configuration parameters requiring a database system restart are heavy. All other parameters are light. Based on those two parameter classes, we map UDO instances into a ``two-level'' MDP, as described next.

\begin{definition}\label{def:heavymdp}
Given an instance of the UDO problem, the \textbf{Heavy Parameter UDO MDP} is an episodic MDP characterized by a tuple $\mdp_H \triangleq \langle \mathcal{S}_H,\mathcal{A}_H,\mathcal{T}_H,\mathcal{R}_H,\mathcal{S}_{DH},\mathcal{S}_{EH}\rangle$. \revision{Here, a state represents a configuration of heavy parameters, i.e. $\mathcal{S}_H \subseteq C_H$.} $\mathcal{S}_{DH}$ and $\mathcal{S}_{EH}$ are start and end states. Compared to Definition~\ref{def:level1mdp}, actions and transitions are restricted to the ones related to heavy (as opposed to light) parameters. The reward function, $\mathcal{R}_H$, is based on the performance metric $f:C\mapsto\mathbb{R}$ of the underlying UDO instance, such that $\mathcal{R}_H \triangleq f_H: C_H \mapsto \mathbb{R}$ with $f_H(c_h)=\arg\max_{c_l\in C_l}f(c_h\circ c_l)$ (i.e., we evaluate a heavy parameter configuration using the optimal, associated light parameter settings).
\end{definition}

\begin{example}
Consider two heavy tuning parameters associated with index creations, i.e.\ parameters $i_1$ and $i_2$, and a light parameter $w$, representing the amount of working memory. Here, the heavy MDP is constituted of four states associated with different index combinations, and actions for adding or removing indices. To evaluate the reward function for a given index configuration, we use the optimal setting for parameter $w$ (or, in practice, an approximation of it). With that setting, we evaluate the benchmark metric (e.g., throughput) on the benchmark workload.
\end{example}

To evaluate heavy parameter settings, we ideally need optimal, associated light parameter settings. The best settings for light parameters depend on the settings for heavy parameters. Now, we formalize light parameter optimization as an MDP to be able to use RL.

\begin{definition}\label{def:lightmdp}
Given an UDO instance and heavy parameter configuration $c_h$, the \textbf{Light Parameter UDO MDP} is an episodic MDP, described by $\mdp_L[c_h] \triangleq \langle\mathcal{S}_L,\mathcal{A}_L,\mathcal{T}_L,\mathcal{R}_L[c_h],\mathcal{S}_{DL},\mathcal{S}_{EL}\rangle$. \revision{Here, $\mathcal{S}_L$ consists of states which are the configurations of light parameters (i.e. $\mathcal{S}_L \subseteq C_L$).} Similarly, $\mathcal{A}_L$ and $\mathcal{T}_L$ represent configuration actions and transitions, restricted to light parameters. The performance for specific light parameter settings depends on the heavy parameter settings. Hence, the reward function $\mathcal{R}_L[c_h]$ is instantiated for specific heavy parameter settings $c_h$ and performance metric $f$, such that $\mathcal{R}_L[c_h] \triangleq f: c_h \times C_L \rightarrow \mathbb{R}$. 
\end{definition}

As shown above, we model optimization for light parameters as a family of MDPs, where each MDP is associated with a specific heavy parameter configuration. Our problem model assumes that only the reward function (i.e., performance) depends on heavy parameters. It is possible to extend the definition above to cover cases where admissible values for light parameters depend on currently chosen heavy parameters. In that case, states, transitions, and actions must be instantiated for specific heavy parameter settings as well. The following example illustrates the interplay between heavy and light parameter MDPs.

% \begin{example}
% Assume our search space is defined by the parameters $\{I_1, I_2, O_1, O_2\}$ with associated discrete value domains. $I_1$ and $I_2$ representing decisions as to whether index one and two are created or not. Parameters $O_1\in\{0,\ldots,7\}$ and $O_2\in\{0,\ldots,4\}$ represent alternative query orderings (identified by an integer number) for transactions one and two. Here, $I_1$ and $I_2$ should be classified as heavy parameters (as creating indexes typically takes time) while $O_1$ and $O_2$ are light (changing query order merely requires switching to a different version of the transaction code). Hence, our search space \revision{$\mathcal{S}_H\triangleq I_1 \times I_2$} for the heavy parameter UDO MDP (level 1) has four states that corresponds to the admissible value combinations for $I_1$ and $I_2$. Its actions $\mathcal{A}_H$ refer only to changes with regards to the indexes. For each index combination, we introduce a separate light parameter UDO MDP (level 2) to optimize settings for \revision{$O_1 \times O_2$}. Thus, there are four light parameter UDO MDPs, and each of them has $7\cdot 4=28$ states. The reward of an index combination (level 1) is calculated based on the (near-)optimal, index-specific settings of $O_1$ and $O_2$. To find those near-optimal settings, the associated MDP at level 2 is solved. Following this, the solutions of level 2 are used to solve the heavy parameter MDP at level 1.
% \end{example}


\tikzstyle{hstate}=[rectangle, fill=blue!10]
\tikzstyle{lstate}=[rectangle, fill=green!10]
\tikzstyle{transition}=[->, black, thick]
\tikzstyle{mapping}=[->, black, thick, dashed]

\begin{figure}
    \centering
    \begin{tikzpicture}
        % Heavy configuration states
        \node[hstate] (root) at (0,0) {$\langle0,0,?\rangle$};
        \node[hstate] (hstate1) at (-3,0) {$\langle1,0,?\rangle$};
        \node[hstate, fill=red!50] (hstate2) at (3,0) {$\langle0,1,?\rangle$};
        % Light configuration states
        \node[lstate] (l1) at (-3,-1) {$\langle1,0,2MB\rangle$};
        \node[lstate] (l2) at (-3,-2) {$\langle1,0,10MB\rangle$};
        \node[lstate, fill=red!50] (l3) at (-1,-1) {$\langle1,0,25MB\rangle$};
        \node[lstate] (l4) at (-1,-2) {$\langle1,0,50MB\rangle$};
        \node[lstate] (l5) at (3,-1) {$\langle0,1,2MB\rangle$};
        \node[lstate] (l6) at (3,-2) {$\langle0,1,10MB\rangle$};
        \node[lstate] (l7) at (1,-1) {$\langle0,1,25MB\rangle$};
        \node[lstate, fill=red!50] (l8) at (1,-2) {$\langle0,1,50MB\rangle$};
        % Heavy transitions
        \draw[transition] (root) -- (hstate1);
        \draw[transition] (root) -- (hstate2);
        % Light transitions
        \draw[transition] (l1) -- (l2);
        \draw[transition] (l1) -- (l3);
        \draw[transition] (l1) -- (l4);
        \draw[transition] (l5) -- (l6);
        \draw[transition] (l5) -- (l7);
        \draw[transition] (l5) -- (l8);
        % Mappings
        \draw[mapping] (hstate1) -- (l1);
        \draw[mapping] (hstate2) -- (l5);
    \end{tikzpicture}
    \caption{Extract of heavy (top) and light (bottom) parameter MDPs for a space with two heavy and one light parameter. Optimal states for each MDP are marked up in red.}
    \label{fig:mdp}
\end{figure}

\begin{example}
Figure~\ref{fig:mdp} illustrates \revision{part of a} two-level MDP. In the illustrated scenario, the configuration space contains two heavy parameters (e.g., index creation decisions) as well as one light parameter (e.g., the maximal amount of main memory used per operator). Rectangles represent states in the figure and are annotated with configuration vectors (reporting parameter in the aforementioned order). The upper part of the figure illustrates the heavy parameter MDP (note that the light parameter is not specified). Solid lines mark transitions due to actions changing the configuration. Dashed lines mark mappings between heavy parameter states and the start state of the associated light parameter MDP. \revision{As index-related parameters are binary, the heavy parameter MDP has four states (out of which three are shown).} In total, the figure illustrates three MDPs (the one for heavy parameters and light parameter MDPs for two heavy configurations). Optimal states are marked up in red, showing that the optimal settings for light parameters may depend on the heavy parameter settings. Identifying optimal settings for heavy parameters requires obtaining optimal, associated settings for light parameters first.
\end{example}

==> sections/new_experiments.tex <==



\input{fig/tpch_performance_sf10}

\input{fig/tpch_space_plus_time}

\input{fig/index_recommendation}

\input{fig/tpch_dynamic}



==> sections/overview.tex <==
\section{System Overview}
\label{sec:overview}



Figure~\ref{fig:overview} shows an overview of the UDO system.  In this section, we discuss UDO's components in detail.

\input{fig/overview}

\subsection{Input and Output}

The input to UDO is threefold. First, we specify a search space for tuning. The search space is defined as a set of tuning parameters that may represent system parameters, physical design choices, or query planning decisions. Each parameter is associated with a set of admissible values and scripts that change the value (e.g., by creating an index). Second, UDO is given a workload to optimize. The workload is represented by a script that evaluates a given configuration with a workload sample and returns a reward value. The reward can represent throughput or the inverse of execution time. Third, UDO obtains a time limit for optimization. The output is the best configuration found until that timeout.

\subsection{Search Space Analysis}

%\textbf{Search Space Analysis.}
Search space analysis examines the space for configuration optimization. In particular, it divides tuning parameters into ``heavy'' and ``light'' parameters. For heavy tuning parameters, changing the value causes non-trivial overheads. Typically, index creations or parameter changes that require restarting the database server are heavy. On the other side, light parameters include system parameters that can be changed without restart or optimizer planning decisions. Here, values can be changed with high frequency. As outlined in more detail next, heavy and light parameters are treated differently during optimization. Currently, we classify parameters based on parameter type, considering parameters related to physical design and parameters requiring database server restarts for changes as heavy, and the others as light. % During analysis, parameters are classified either based on parameter type or based on a test measuring time for value changes.

Next, the search space analyzer creates an environment in which learning takes place. UDO uses reinforcement learning as core optimization mechanism. Reinforcement learning generally applies to Markov Decision Processes (MDPs), defined by states, actions, state transitions, and a function that assigns transitions to reward values. Here, we associate actions with configuration changes (e.g., creating an index or changing a system parameter). States are associated with configurations. Actions transition from a state representing a first configuration to a state representing the configuration obtained, after applying the change represented by the action to the first configuration.

As discussed in more detail in Section~\ref{sec:model}, a particularity of our approach is that we divide the search space into two levels. The top level is focused on heavy parameters alone. Each state only represents choices for those parameters and actions refer only to those parameters. The reward for taking an action in a state is linked to the performance improvement obtained by the associated configuration change. The performance depends however not only on choices for heavy parameters but also on choices for light parameters. Ideally, we want to assess settings for heavy parameters, based on the optimal settings for the light parameters. The optimal settings for light parameters may however depend on the choices for heavy parameters (e.g., we may want to disable sequential scans in the optimizer search space only after creating a particularly useful index). Hence, we introduce a second level of optimization that focuses on light parameters only. Here, we assume fixed values for heavy parameters while exploring a state space representing alternative settings for light parameters. As outlined next, this separation enables us to reduce overheads related to configuration changes. The search space analyzer creates an implicit representation of search space (i.e., we avoid representing a large search tree explicitly), which is used to initialize the reinforcement learning agents.


\subsection{Reinforcement Learning}

%\textbf{Reinforcement Learning.} 
UDO applies reinforcement learning to solve the MDPs described before. As discussed before, we decompose the search space into multiple dependent MDPs. Doing so allows us to solve those MDPs by different algorithms. We outline next why that is interesting.

Reinforcement Learning (RL) often benefits from a high frequency of iterations. This allows the RL agent to explore the search space in depth within a reasonable time frame. In our case, iteration frequency is limited by two factors: \textit{time for creating a configuration} and \textit{time for evaluating a configuration}. The time for evaluating a configuration can often be reduced via sampling (from the given workload). As we consider stochastic rewards in general, obtaining performance on a sample is in principle sufficient for convergence. The time for creating configurations, however, cannot easily be reduced. For instance, actions related to physical design changes (e.g., index creations) can take significant amount of time. As we cannot fully avoid such overheads, \textit{our goal is to amortize them over multiple evaluations} instead.

For instance, to decrease index creation overheads per iteration, we ideally want to create indexes once and then evaluate a set of similar configurations consecutively. Standard RL algorithms do not comply with this requirement. They expect reward values immediately after taking an action. This does not leave any slack to collect similar configurations before evaluating them. Hence, specifically for the MDP optimizing heavy parameters, we use algorithms that accept delays between taking an action and obtaining the associated reward~\cite{Joulani2013a}. We propose a corresponding algorithm in Section~\ref{sec:rlalgs} and analyze its convergence properties in Section~\ref{sec:analysis}.  %\deba{have to add a line on delayed uct here}

%the Delayed Online Learning algorithm ~\cite{joulani2013online,li2019bandit}. This algorithm works for scenarios in which reward values become available with a delay. 

Instead of evaluating heavy parameter configurations directly, we forward them to the evaluation manager component. This component, described in the next subsection, uses cost-based planning to evaluate configuration sets efficiently. Once performance results become available, the corresponding reward values are forwarded to the RL agent. We use an algorithm that copes with delayed rewards to optimize heavy parameters. On the other side, we use no-delay RL algorithms, specifically the Hierarchical Optimistic Optimization (HOO) algorithm~\cite{bubeck2011a} with Rapid Value Estimation~\cite{Gelly2007a}, to optimize light parameters. Since changes are cheap, amortization is not required here, and it would only delay convergence unnecessarily. We show in Section~\ref{sec:experiments} the practical benefits of this two-level approach.

%\textbf{Evaluation Manager.} 
\subsection{Evaluation Manager}

The evaluation manager (short: evaluator) continuously receives evaluation requests from the RL agent. Each evaluation request refers to a configuration whose performance has to be evaluated. Additionally, each request specifies a deadline until which the evaluation result is required. The evaluation manager is responsible for addressing each request before the deadline. Under that constraint, its goal is to minimize evaluation overheads. Such overheads are minimized by optimizing the point in time and the order in which configurations are evaluated. 

More specifically, we focus on minimizing overheads for creating configurations to evaluate. For instance, we amortize index creation overheads if we evaluate two configurations with similar indexes consecutively. We amortize overheads for a database server restart (to have system configuration parameter changes take effect) if we evaluate multiple configurations using the current settings consecutively. The evaluation manager tries to take advantages of such effects as much as possible. Sections~\ref{sec:evaluation} and \ref{sec:picking} describe the evaluation manager in more detail. 

%describes the process according to which the evaluator chooses the configurations to evaluate within a specific time slot. 


%\textbf{Evaluation Planner.} 

\subsection{Evaluation Planner}

In order to reduce overheads, the evaluation manager uses a cost-based planner. This planner formalizes the evaluation of configuration sets as an optimization problem. The goal is to minimize overheads for switching between configurations while generating all results until the corresponding deadline.

The cost model of the planner is based on time measurements, taken when changing heavy parameters. The search space corresponds to configuration evaluation orders that are admissible, given the current evaluation deadlines. To explore this search space, the planner uses either integer programming or, for large problem instances, a cheaper, greedy approach. Both approaches are described in detail in Section~\ref{sec:ordering}.

% The dynamic programming algorithm adopts a bottom-up approach, it iterates the power set. it considers the power set of reorder unit, and iterates those sets and calculate the best order as increasing cardinaility from 1 to $n$. 

% The dynamic programming algorithm adopts a bottom-up approach, it considers the power set of reorder unit, and iterates those sets and calculate the best order as increasing cardinaility from 1 to $n$. 

% The algorithm uses the best order for sets with cardinality less than $n$ to calculate the best order for sets with cardinality $n$.

% We formalize our plan problem as follows, given the maximal delay deadline time $\Delta t$, at each timestamp $t$, we receive a configuration $c_t$ generated by search trees and decide which configurations are evaluated at the current stage (notice that the configurations generated at timestamp $t - \Delta t$ must be evaluated. We consider both online algorithm and offline algorithm to solve this problem. 

% \paragraph{Offline algorithm} We simplify the previous procedure to the following offline procedure, instead deciding which configurations to evaluate, we gather configurations for the continuous timestamps $\Delta t$, and find the min cost order for all those heavy configurations. For example, the RL algorithm generates configurations $C = \{ c_0, c_1, \cdots, c_{\Delta t} \}$ from timestamp $t = 0, 1, \cdots, \Delta t$. Our goal is to find a permutation of configuration set $C$, denoted as $\bar{C} = \{ \bar{c}_0, \bar{c}_1, \cdots, \bar{c}_{\Delta t} \}$, such that the total cost of $\bar{C}$, which is $\sum_{t=0}^{\Delta t} \bar{c}_t - \sum_{t=0}^{\Delta t - 1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$ is minimized. This problem is same as maximizing the overlapping cost,  $\sum_{t=0}^{\Delta t - 1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$. This problem can be proved a NP-complete problem by reducing it to the Hamiltonian path problem. We propose a dynamic programming algorithm. We formula it as an integer programming problem as follows, we use $x_{ij}$ to denote the $i$-th unit is reordered to the $j$-th place. 

% \begin{equation*}
% \begin{array}{ll@{}ll}
% \text{maximize}  & \displaystyle
% \sum_{i=1}^{\Delta t} 
% \sum_{j=1}^{\Delta t - 1}
% \sum_{k=1}^{\Delta t} z_{ijk}
% \text{cost}(c_{i} \cap c_{k}) 
% &\\
% \text{subject to}& 
% \displaystyle z_{ijk} \leq \frac{1}{2} (x_{ij} + x_{k (j+1)}) \\
% & \displaystyle\sum_{i=1}^{\Delta t} x_{ij}  = 1,  &j=1 ,..., \Delta t\\
% & \displaystyle\sum_{j=1}^{\Delta t} x_{ij} = 1,  &i=1 ,..., \Delta t\\
% \end{array}
% \end{equation*}


% \paragraph{Online algorithm}
% The cost-based planner estimates the saving benefit if each pending configuration is evaluate at this time and decides which configurations should be evaluate. We propose an algorithm based on the optimal stopping theory. For each configuration, we split its delay deadline $\Delta t$ into two procedure, training procedure and evaluating procedures. In the training procedure, the planner calculates the saving benefits of the given configuration at each timestamp, and in the evaluating procedure, the planner builds the given configuration at timestamp which gives more benefit than the best benefit obtained in the training procedure.

% Our algorithm always chooses not to evaluate the configurations until we reach to the timestamp $t - \Delta t_1$, where $t$ is the generated timestamp of given configuration and $\Delta t_1$ is a subinterval of $\Delta t$. And we collect the best saving cost in this subinterval, and 

% and $\text{cost}$ is a function mapping from specific configurations to their build/drop costs.


==> sections/planning.tex <==
\subsection{Optimizing Evaluation Order}
\label{sec:ordering}

Given a set of configurations to evaluate, we can influence cost via the evaluation order. For instance, if we evaluate configurations with similar indices consecutively, we can reduce associated index creation costs. Our goal is to find evaluation orders that minimize re-configuration overheads. \revision{We introduce the problem formally.} 

\color{red}
\begin{definition}\label{def:orderingproblem}
An instance of \textbf{Reconfiguration Cost Minimization} is defined by a set $R=\{r_i\}$ of requested (heavy parameter) configurations to evaluate and a cost function $\mathcal{C}:R\times R\mapsto\mathbb{R}^+$ that maps a pair $r_1$, $r_2$ of requested configurations to the cost for switching from $r_1$ to $r_2$ (e.g., by creating indexes that appear in $r_2$ but not in $r_1$). A solution is a permutation $\Pi:\mathbb{N}\mapsto R$ of configurations, representing evaluation order with cost $\sum_i\mathcal{C}(\Pi(i),\Pi(i+1))$. An optimal evaluation order minimizes cost.
\end{definition}
\color{black}

% such that the cost of evaluating of configurations The Reconfiguration problem is defined, given a configuration list $C_h = \{ c_1, c_2, \cdots, c_l \}$ with length $l$ and a cost metric $c_{i,j}$ indicating the cost of switching from configuration $i$ to configuration $j$, the goal is to find a permutation function $\Pi$ that maps positions from 1 to $l$ to indices from 1 to $l$, to minimize the total Reconfiguration cost, $\sum_{1\leq i<l}c_{\Pi(i),\Pi(i+1)}$.

% denoted as $\bar{C} = \{ \bar{c}_1, \bar{c}_2, \cdots, \bar{c}_l \}$, such that the total cost of $\bar{C}$, $\sum_{t=1}^{l} \bar{c}_t - \sum_{t=1}^{l-1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$ is minimized. This problem is same as maximizing the overlapping cost, $\sum_{t=1}^{l - 1} \text{cost}(\bar{c}_t \cap \bar{c}_{t+1})$.

% Let's just use generic cost constants c_{i,j} indicating the cost of switching from configuration i to configuration j - in general, introduce only as much formalism as necessary. You can just optimize a permutation function that maps positions from 1 to l to indices from 1 to l, then \sum_{1\leq i<l}c_{\Pi(i),\Pi(i+1)} gives you the cost.

% We show in Section~\ref{sec:analysis} that this problem is NP-hard.

\revision{In the current implementation, we approximate $\mathcal{C}(r_1,r_2)$ by only considering indexes that appear in $r_2$ but not $r_1$ and summing up the cardinality of the indexed table over all added indexes.} Next, we analyze the computational complexity of this problem (called ``reconfiguration cost minimzation'' in the following). 


%\vspace{-0.9em}
\begin{theorem}
Reconfiguration cost minimization is NP-hard.
\end{theorem}
%\vspace{-2.3em}
\begin{proof}
\label{pf:reconfiguration}
Consider an instance of the Hamiltonian graph problem. This instance is described by a graph $G$, the goal is to construct a path visiting each node once. We reduce to reconfiguration cost minimization as follows. For each node $i$ in $G$, we introduce one evaluation request $r_i$. For each pair of nodes $i$ and $j$, connected by an edge in $G$, we set the reconfiguration cost $\mathcal{C}(r_i,r_j)$ to zero, otherwise to one. Assume we find an evaluation order with a reconfiguration cost of zero. In this case, we obtain a Hamiltonian path in the original problem instance (visiting nodes, associated with requests, in the order in which requests are selected for evaluation). As each request is evaluated once, the associated graph node is visited once. As the reconfiguration cost is zero, all visited nodes are connected by edges.
\end{proof}

%\begin{proof}We reduce this problem to Hamiltonian path problem. Given a graph $G$ of $n$ vertices and a minimal cost re-configuration solver, we represent each vertex $i$ of the graph $G$ to one configuration set $c_i$. And if there exist one edge between vertex $i$ and $j$, we construct the set $c_i$ and $c_j$ which have one overlap configuration. And if there does not exist one edge between vertex $i$ and $j$, the constructed set $c_i$ and $c_j$ does not have any overlap configurations. Then we generate a list of configurations $\{c_0, c_1, \cdots, c_n\}$ using the given graph. Then we feed this configuration list into our minimal cost re-configuration solver with the cost function mapping each configuration to one unit overhead. Then we obtain a permutation order of the configuration list $C$. We traverse the graph with the obtained vertex order. If the graph exists a Hamiltonian path, the path using the obtained vertex order must be one Hamiltonian path. Otherwise, the graph does not exist any Hamiltonian path. \end{proof}
% If we succeed to generate a path finally, the generated path is a valid Hamiltonian path, otherwise the graph does not exist any Hamiltonian path. 
% using this obtained order, if we succeed to generate a path finally, the generated path is a valid Hamiltonian path, otherwise the graph does not exist any Hamiltonian path. 
%\vspace{-1.5em}

Hence, we must choose between efficient optimization and guaranteed optimal results. In the following, we present a greedy and an exhaustive algorithm to solve this problem.

\subsection{Greedy Algorithm}

\begin{algorithm}[t!]
\caption{\textproc{PlanConf}: Order configurations for evaluation.}
\label{alg:greedyPlan}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} Evaluation requests $R$
\State \textbf{Output:} Requests in suggested evaluation order
\Function{PlanConf-Greedy}{$R$}
\State \Comment{Initialize list of ordered requests}
\State $O\gets[]$
\State \Comment{Iterate over all requests}
\For{$r\in R$}
\State \Comment{Find optimal insertion point}
\State $i\gets\arg\min_{i\in 0,\ldots,|O|}C_R(O[i-1],O[i])+C_R(O[i],O[i+1]))$
\State \Comment{Insert current request there}
\State $O.insert(i,r)$
\EndFor
\State \Return{$O$}
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

Algorithm~\ref{alg:greedyPlan} generates evaluation orders via a simple, greedy approach. The input is a set of evaluation requests (each one referencing a configuration to evaluate). Starting from an empty list, we expand the evaluation order gradually, by adding one more request in each iteration. We insert each request greedily at the position where it leads to minimal reconfiguration overheads. We measure re-configuration overheads via function $C_R(c_1,c_2)$, measuring reconfiguration overheads to move from configuration $c_1$ to configuration $c_2$. Those overheads include for instance index creation overheads for indices that appear in $c_2$ but not in $c_1$. After identifying the position with minimum overheads, we expand the order accordingly.

\subsection{Integer Programming}

Next, we show how to transform the problem of ordering evaluations into an integer linear program. After doing so, we can use corresponding solvers to find an optimal solution quite efficiently. Our decision variables are binary: we introduce variables $e_t^r$ to indicate whether request $r$ is evaluated at time $t$. We introduce variables for each request $r\in R$ to evaluate and for $|R|$ time steps. We evaluate one configuration at each time step, represented by constraints of the form $\sum_{r}e_t^r=1$ (for each time step $t$). Also, we must evaluate each configuration once which we represent by the constraint $\sum_{t}e_t^r=1$ (for each request $r$)\footnote{Strictly speaking, the last constraint is redundant as we evaluate exactly one configuration in each times step.}. The objective function is determined by reconfiguration costs. For each pair of configuration requests $r_1$ and $r_2$, we can estimate reconfiguration cost $C_R(r_1,r_2)$ by comparing the associated configurations. We introduce binary variables of the form $i_t^{r_1,r_2}$, indicating whether reconfiguration costs for moving from $r_1$ to $r_2$ is incurred at time $t$. We introduce those variables for each pair of configurations and for each time step. The objective function is given as $\sum_{t,r_1,r_2}c_R(r_1,r_2)\cdot i_t^{r_1,r_2}$ (our goal is to minimize this function). Lastly, we need to ensure that the value assignments for variables $i_t^{r_1,r_2}$ and $e_t^r$ are consistent. Due to the objective function, variables $i_t^{r_1,r_2}$ will be set to zero if possible. Hence, we only must constrain them to one if the context requires it. We do so by introducing constraints of the form $i_t^{r_1,r_2}\geq (e_t^{r_1}+e_{t+1}^{r_2})/2$ for each pair of requests and for each time step. The optimal solution to this linear program describes an optimal evaluation order.

==> sections/scheduling.tex <==
\subsection{Picking Configurations to Evaluate}
\label{sec:picking}

\begin{algorithm}[t!]
\caption{\textproc{PickConf}: Methods for picking configurations to evaluate.}
\label{alg:pickConfigurations}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \textbf{Input:} Evaluation requests $R$, current timestamp $t$
\State \textbf{Output:} Set of configurations to evaluate
\Function{PickConf-Threshold}{$R,t$}
\State \Comment{Was size threshold reached?}
\If{$|R|\geq\rho$}
\State \Comment{Return all requests}
\State \Return{$R$}
\Else
\State \Return{$\emptyset$}
\EndIf
\EndFunction
\vspace{0.15cm}
\State \Comment{Initialize maximal cost savings for each request}
\State $S=\emptyset$
\vspace{0.15cm}
\State \textbf{Input:} Evaluation requests $R$, current timestamp $t$
\State \textbf{Output:} Set of configurations to evaluate
\Function{PickConf-Secretary}{$R,t$}
\State \Comment{Add requests whose deadline is reached}
\State $E\gets \{\langle c_H,t_D\rangle\in R|t_D\geq t\}$
\State \Comment{Remove requests from pending set}
\State $R\gets R\setminus E$
\State \Comment{Iterate over requests}
\For{$r=\langle c_H,t_D\rangle\in R$}
\State \Comment{Calculate re-configuration cost savings}
\State $s\gets$\Call{CostSavings}{$r,E$}
\State \Comment{Retrieve maximal savings so far}
\State $m\gets S(r)$
\State \Comment{Should we evaluate?}
\If{$t-(t_D-\delta)\geq\delta/e\wedge s>m$}
\State $E\gets E\cup\{r\}$
\EndIf
\State \Comment{Update maximally possible savings}
\State $S(r)\gets\max(m,s)$
\EndFor
\State \Return{$E$}
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

The evaluator can decide, within certain boundaries, when to evaluate configurations. Evaluating configurations in batches of similar configurations is often cheaper. It is often possible to amortize re-configuration overheads over multiple, similar configurations. Hence, to decide when to evaluate, the evaluator may take into account the set of pending evaluation requests.

We present two strategies for selecting configurations to evaluate. Algorithm~\ref{alg:pickConfigurations} shows corresponding pseudo-code. The two functions represented in Algorithm~\ref{alg:pickConfigurations} (Function~\textproc{PickConf-Threshold} or \textproc{PickConf-Secretary}) implement the call in Line~12 of Algorithm~\ref{alg:evalVar}. Next, we discuss the two strategies in more detail.

The first strategy, represented by Function~\textproc{PickConf-Threshold}, is relatively simple. We select all pending evaluation requests for processing if their number has reached a threshold. This threshold is represented as parameter $\rho$ in the pseudo-code. Before reaching the threshold, we simply collect evaluation requests without actually processing them (i.e., the set of selected requests is empty). By evaluating requests in batches, we hope to amortize re-configuration overheads via the planning mechanisms outlined in the next section. The threshold $\rho$ is a tuning parameter. It is associated with a tradeoff. Choosing $\rho$ too small reduces chances for cost amortization. Choosing $\rho$ too large means that we introduce significant delays for the RL algorithm between a configuration is selected and evaluated. Delaying feedback may increase time spent in exploring uninteresting parts of the search space. Note that $\rho$ must be smaller or equal to the maximal delay, allowed by the RL algorithm. In our experiments, we typically set $\rho$ to 20. Empirically, we determined this setting to work well for many scenarios. 

Our second strategy, written as Function~\textproc{PickConf-Secretary}, is more sophisticated and often works better in practice. It is motivated by algorithms for solving the so called ``Secretary Problem''~\cite{Hill2009}. This problem models a job interview for a single position, in which a hiring decision must be made directly after each interview. This decision is hard due to uncertainty with regards to the quality of the remaining candidates. A popular algorithm for this problem reviews a fraction of $1/e$ of candidates without hiring any. Then, it selects the first candidate better than all previously seen candidates (or the last candidate, if no such candidate emerges). It can be shown that this strategy makes a near-optimal choice likely. We use an adaption of this algorithm for our problem.

In our case, candidates correspond to evaluation times for a fixed configuration. The re-configuration cost, required to test a specific configuration, decreases if similar configurations were evaluated before. E.g., we do not have to create an expensive index, part of a configuration to evaluate, if that index was created before. So, instead of immediately evaluating a configuration, we may want to wait until similar configurations are requested. Of course, we cannot know precisely which configurations will be submitted for evaluation in the future. This is akin to the uncertainty about the quality of future job candidates. 

Algorithm~\ref{alg:pickConfigurations} keeps track of possible cost savings for specific configurations. Global variable $S$ keeps track of maximal savings in re-configuration costs for specific configurations, over different invocations of \textproc{PickConf-Secretary}. We compare current cost savings to the maximum seen so far to decide when to evaluate. Intuitively, we want to evaluate configurations in invocations, during which we can obtain particularly high cost savings. 

Function~\textproc{PickConf-Secretary} first selects all evaluation requests whose evaluation deadline has been reached (Line~18). Then, we iterate over the remaining requests. For each request, we calculate re-configuration cost savings, assuming that we evaluate it after the configurations selected for evaluation so far. Next, we retrieve maximal cost savings observed for this configuration so far (Line~26). We select the configuration for evaluation if we have observed cost savings over a sufficiently large period (condition $t-(t_D-\delta)\geq \delta/e$ where $\delta$ is the maximal delay and $e$ Euler's number) and if current savings exceed the previous optimum (condition $s>m$). We show in Section~\ref{sec:analysis} that, under moderately simplifying assumptions, we achieve optimal cost savings per configuration in about one third of cases.

